The Framework Tax: Disparities Between Inference Efficiency in NLP Research and Deployment

Increased focus on the computational efficiency of NLP systems has motivated the design of efficient model architectures and improvements to underlying hardware accelerators. However, the resulting increases in computational throughput and reductions in floating point operations have not directly translated to improvements in wall-clock inference latency. We demonstrate that these discrepancies can be largely attributed to bottlenecks introduced by deep learning frameworks. We denote this phenomenon as the \textit{framework tax}, and observe that the disparity is growing as hardware speed increases over time. In this work, we examine this phenomenon through a series of case studies analyzing the effects of model design decisions, framework paradigms, and hardware platforms on total model latency. Code is available at https://github.com/JaredFern/Framework-Tax.

==> sections-emnlp/appx-recipes.tex <==
\section{Efficient Inference Recipes}
We provide the following reference setting for efficient inference: 
\begin{itemize}
    \item Mixed Precision
    \item Layer Fusion
    \item Sparsity 
    \item CUDA Graph
\end{itemize}

==> sections-es/1-intro.tex <==
\section{Introduction} 
     Machine learning efficiency is especially important in inference settings when models are used repeatedly and at scale. For example, Meta reports that inference workloads make up 70\% of their AI power consumption, with the remaining 30\% due to training and development \citep{wu2022sustainable}, while Google attributes 60\% of their ML energy consumption to inference \citep{patterson2022carbon}. Inference is also estimated to make up 80 to 90\% of ML cloud computing demand \cite{barr2019amazon, leopold2019aws}. 
    
    \begin{figure}
        \centering
        \includegraphics[width=0.35\textwidth]{assets/assets-1/figure-1.pdf}
        \vspace{-5pt}
        \caption{Latency as a function of a model’s multiply accumulate operations (MACs) with PyTorch on an NVIDIA 2080ti GPU. Expected relationships do not hold; model complexity and hardware capabilities fail to predict latency due to framework-boundedness.}
        \label{fig:fig1}
        \vspace{-15pt}
    \end{figure}    

    These concerns have spurred innovations in efficient model architecture design with lesser computational requirements, that reduce number of model parameters and multiply-accumulate operations (MACs) \cite{tan2019efficientnet, dai2020funnel, sun2020mobilebert}. Likewise, improvements to GPU hardware accelerators applications have seen similar performance gains with the number of floating point operations per second (FLOPS) growing by over 175\% in the past 5 years. Despite this progress, the supposed gains offered by faster hardware and more efficient models are often not realized in deployment settings, where model speed has not improved as seen in Figure \ref{fig:fig1}.

    This misalignment is primarily attributable to overhead incurred by the machine learning frameworks used to implement and execute neural network models. As a manifestation of Amdahl's Law in machine learning systems, we see that despite increases in hardware speeds, the overhead introduced by commonly used deep learning frameworks during kernel dispatch operations is non-negligible and imposes bottlenecks on overall execution time. 
    We refer to this phenomena as the \textit{framework tax}, and show that it exists across deep learning framework paradigms (e.g. eager execution, just-in-time, and ahead-of-time compilation). Due to fixed framework overhead that dominates the execution at small batch sizes, proxy measurements of model efficiency, such as MACs and parameter count, are not predictive of inference latency.
    % Furthermore, we note that existing efforts to improve model efficiency by designing faster GPU kernels do not reduce latency, when total execution is still bound by fixed framework overhead. 
    Moreover, as hardware performance increases and reduces the time for computational graph execution, machine learning systems are \textit{increasingly} framework-bound at larger batch sizes. 
    
\vspace{8pt}

    We identify common decisions that emerge in during the design of efficient model architectures, inference environments, and hardware accelerators and isolate choices likely to mislead a practitioner. We analyze the performance of convolutional neural networks (CNNs) and transformer models in eager execution PyTorch, just-in-time compiled TorchScript, and an ahead-of-time compiled ONNX runtime. We perform our study across seven different GPUs from the Pascal, Turing, and Ampere Nvidia GPU microarchitectures. We provide a series of recommendations for ML researchers and practitioners presented through a collection of case studies.
    % Among these, we argue for increased usage of inference runtimes in small batch size settings as they observe substantially less framework overhead. Alternatively, when using eager execution-based frameworks for inference, we recommend increasing model width or batch size to take advantage of increased model capacity. 
    % For example, hidden dimensions in self-attention and fully connected layers can be doubled to increase model capacity without affecting latency, implying that model designers have an extra degree of freedom often overlooked when designing around parameters or FLOPs.
    % We hope that our analysis and recommendations will help bridge the gap between efficient ML research and practice.
    
    % Alternatively, we recommend increasing model width or batch size for inference with eager execution-based frameworks that have larger per-layer overhead to take advantage of increased model capacity at no cost to latency. 
    
     % We confirm existing observations that hardware and implementation support result in differing peak rates of computation for different arithmetic operations \cite{cai2018proxylessnas, sandler2018mobilenetv2}. As seen in Figure~\ref{fig:MacsLatency}, we observe that as hardware speed increases model latency is no longer a function of the amount of computation being performed.
     
    % However, these commonly used efficiency cost indicators often correlate poorly with direct measurements of model performance, as seen in Figure~\ref{fig:MacsLatency} -- observing that FLOPs is a poor predictor of latency. These measures are intrinsic to a model's architecture and are oblivious to the supporting framework and hardware. As a result, they ignore infrastructure details that are important in predicting a model's actual performance when deployed in practice, such as the management of kernel launches, the sequential structure of the computational graph, and the supported parallelism of underlying hardware. Optimization of model architecture design towards these metrics potentially misleads the ML community into designing purportedly efficient models that fail to meet latency requirements when deployed in practice and generalize poorly to other hardware.

    % Software advances have been developed independently of hardware leading to mismatch in utilization
    % In this work, we systematically evaluate the impact of model architecture, framework and hardware platform on model latency in the inference setting. We examine how different approaches to efficient model design impact wall-clock latency. We examine how different framework paradigms (e.g. eager execution, just-in-time and ahead-of-time compilation) can be used to accelerate model execution. We observe that the software frameworks used to implement and execute neural networks introduce bottlenecks to inference latency, and introduce the new metric of \textbf{framework overhead} to quantify this property.



% (1) peak rate of computation is dependent on the type of arithmetic operation being performed, (2) density of arithmetic operations is inconsistent across layers, (3) sequential dependencies in a neural network model's computational graph limit the degree to which hardware parallelism can be exploited. These properties lead each neural network architecture to exhibit different levels of compute and memory boundedness for a given hardware. Motivated by these insights, we develop a systematic method for evaluating the impact of model architecture, deep learning framework, and hardware platform on model latency. 

% Using these insights, we discuss how alignment of parallelism between model architecture and hardware, software platforms can be best leveraged to increase throughput and hardware utilization. We discuss model design implications and pareto-optimal scaling of model hyperparameters such as layer width.

% As seen in Figure \ref{fig:MacsLatency}, we verify existing results that while number of MACs are a reasonable proxy for speed on CPU-based devices, it is poor indicator of model speed on parallel core architectures. In section \ref{section:flops-util}, we show that this misalignment can be attributed to two main factors: different operations having differing FLOP utilization, model architecture imposing dependency bottlenecks that limit parallel computation. In section \ref{section:roofline}, we show that all models are in fact both memory and compute bound depending on the size of input and number of per-layer FLOPs. In section \ref{section:latency}, we show that the factors that effect model speed in each regime and propose a more comprehensive model for latency estimation. 


% High-Level Goal: Fast and Performant Models
%	- High expressivity: Deeper models, and more parameters per layer
% 	- Low Latency, Throughput: Cheap or Fewer operations 
% 1. Parallellism lets us beat FLOPs as a metric; 
% 	- Not all FLOPs are the same
% 		- Some operations are more expensive
%		- Overhead and underutilized parallelism negates the cost of increased FLOPs 
% 2. Inference compute landscape is complicated by the structure of the underlying hardware
% 	- Memory Bound vs Compute Bound
% 3. 

% Meanwhile, efforts to benchmark hardware and software platforms target fixed  reference models and workloads, leading to the development of custom hardware platforms and compute kernels.  
% Fixed is not entirely true

% There exists a disconnect between the 
% Guidance:
%     - Frameworks: Reduction in the overhead; Speedups are obtainable through layer fusion and serialization

% Motivation: Real-world throughput and latency is an important dquality of neural network models. 
%     - Deployment of edge and specific use-case modeling is a case for hardware-software codesign; i.e. Understand how well a model architecture leverages its target hardware platform
%     - Neural Architecture Search learns these properties implicitly but inefficiently 
%     - Continuous Latency Constraints are not representative of underlying system behavior

% Research Questions
% 0. Question: What determines the actual latency of a model
% 1. Question: How does one determine the overhead of a model? Why do models differ in their roofline heights?
%     - Hardware Support: 
%         - Computation parallelism
%     - Model and Platform properties:
%         - Easy Cases:
%             1. Computational Complexity is Constant throughout the model and it saturates together
%             2. Computational Complexity is Dominated by a Single Operation 
%         - Hard Case: 
%             1. Multiple and Staggered Bottlenecks -- Majority of Computation is not in the "most complex" operation, i.e. DenseNet
%             2. Average latency 
% 2. Question: When does a particular model architecture saturate its compute resources?
%     A. Compute boundedness is dependent on the saturation of operations
%         A1. Bottlenecks for a single model architecture is primarily dependent on operation selection and support

% 3. Can we apply a transformation or model f(hardware, architecture/operation) to determine relatively when operations saturate?
%     - Per operation: 

% Proposals:
% 1. Parallelized Latency is non-linear piecewise:
%     - Memory, Overhead Bound Regime 
%         - Operation Setup + Teardown + Model, Layer Overhead >> Computational Complexity Time
%     - Operation Saturation Regime
%         - Saturation roughly occurs on a per-layer basis
%             0. Find Saturation Points of Conv2D, MBConv, Linear, BatchNorm2D, LayerNorm
%             1. Equivalence of Different Operations to GEMMs
%         - Proposed Experiment and Case Studies:
%             0. Examine Saturation of Homogeneous Models (ResNet and ViT)
%             1. Examine Saturation of Funnel Transformer
%             2. Examine Saturation of Multimodule Models (Inception Net)
%         - Memory Bandwidth Complexity Increases alongside computational complexity (i.e. Roofline max)
%     - Full Computational Bound, Saturation:
%         - Caveats: CPU Fallback on Large Batch Size
% 2. Determining Saturation on a Platform:
%     - Precision 
% 3. Conclusions: 
%     - Optimal hardware-software single example throughput should optimize under the saturation constraint instead of FLOPs 

% Orthogonal Work
%  - JiT Compilation: Computational 
%  - Mixed Precision: 


% Contributions
% 1. Examination of model architecture and hardware as factors on computational bottleneck
%     - Effects of 
%     - Accross Architecture Paradigms: Transformers and CNNs
% 2. Methodology for determining bottlenecks and Target Latency for NAS results
%     - Reduction in Search Space 
% 3. Not a proxy or hand tuned measure

% Model Development Guidance:
% 1. Any operation in the overhead constrained regime is pareto suboptimal
% 2. 

% Additional Experiments: 



% 2. Decomposing the separations:
%     - Well implemented common operations: MM, Conv2D
%     - Overhead: Python Runtime, Kernel Launches
%     - Poorly Parallelized Implementations: 


% General roofline analysis for neural networks fails because models vary across their archit ectures and their constituent operations. 

% Additionally, the focus on operation throughput does not account for the often more important sample level throughput.


==> sections-es/2-related_work.tex <==
\section{Related Work}
\subsection{Neural Network Frameworks and Runtimes}  
    Specialized frameworks enable execution of deep learning workloads by implementing and providing APIs for tensor operations, gradient calculation, and construction of computational graphs. Frameworks generally fall into the following design paradigms \cite{kahn2022flashlight}:
    % \vspace{-5pt}
    \begin{itemize}[leftmargin=*]
        \item \textbf{Eager Execution}: A computational graph is constructed from a series of operations that are executed as soon as they are called from an interpreter. Examples include: PyTorch \cite{paszke2019pytorch}, TensorFlow 2.0 Eager \cite{tensorflow2015-whitepaper}, Chainer \cite{tokui2015chainer}. 
        \item \textbf{Deferred Execution}: A series of operations are defined and executed on sample data to generate a dataflow graph that can then be just-in-time (JiT) compiled. Examples include: PyTorch TorchScript, Jax \cite{jax2018github}, Theano \cite{al2016theano}, Caffe \cite{jia2014caffe}.
        \item \textbf{Static}: A computational graph is pre-defined, compiled, and executed inside a specialized runtime; allowing for aggressive, global ahead-of-time compiler (AoT) optimizations. Examples include: ONNX Runtime, TensorFlow 1.0, MXNet \cite{chen2015mxnet}, Nvidia TensorRT, and TVM \cite{chen2018tvm}. 
    \end{itemize}

    % \vspace{-10pt}
    While naively, the deferred and static settings appear to provide obvious benefits in production settings -- the machine learning research community continues to rely heavily on eager mode frameworks for their ease of use.  This further exacerbates the community divide, where models are designed under different assumptions than deployed. 
        
    Deferred and static execution frameworks leverage JiT or AoT compilation of their computational graphs allowing for optimizations such as operator fusion. However, they are limited in model expressivity due to reduced support for structures such as control flow and dynamic input sizes. In contrast, models under the eager execution paradigm allow for more flexibility but incur larger amounts of framework overhead running inside an interpreted environment. 


\subsection{Efficiency Metrics \& Efficient Model Design}
        To measure model efficiency, metrics intrinsic to the model architecture are often reported such as the number of trainable parameters, number of floating point (FLOPs) or multiply-accumulate (MACs) operations. Number of trainable parameters is a frequently reported metric as a proxy for memory usage.  However, parameter count is often not predictive of model speed \cite{zhou2020hulk} and techniques such as weight tying can reduce in parameter counts without reducing the amount of computation \cite{lan2019albert}. 

        %Number of FLOPs is a common measure used to evaluate the amount of computation required by a model. 
        Optimizing for FLOP counts has motivated the development of model architectures that achieve comparable task performance under a fixed FLOP budget \cite{dai2020funnel} and scaling model width and depth to reduce overall size \cite{sanh2019distilbert}. Low-FLOP operations, such as grouped convolutions \cite{iandola2016squeezenet, zhang2018shufflenet} and inverted residual bottlenecks \cite{sandler2018mobilenetv2, sun2020mobilebert}, have been developed as substitutes for their standard, dense counterparts.  However, the tensor operation primitives and underlying hardware support varying levels of parallelism for different arithmetic operations, leading to low correlation between FLOPs and latency.

        % From the perspective of device utilization, hardware and model FLOPs utilization are reported as the ratio between observed FLOPs per second and a hardware platforms peak theoretical FLOPs. 
    
        % Finally, Critical Datapath Length (CDL), or model depth, corresponds to the number of required tensor operations in a model \cite{langerman2020beyond}. 
        % CDL assumes that parallelizable layers will be run in parallel -- in practice this rarely holds as layers are executed as separate kernel calls.
        % However, for single example inference, CDL has been shown to have a higher correlation with model latency on GPU than number of FLOPs. Previous work where CDL was tested with Vanilla PyTorch limited analysis to examples of batch size one in the inference setting.
    
        Previous works examining the relationship between the mentioned efficiency measures have shown that these metrics often do not correlate well with each other, nor with direct measurements of latency in large scale training \cite{dehghani2021efficiency, wang2020systematic}. We extend this analysis to this inference setting and show that some of these metrics breakdown entirely due to additional performance bottlenecks that emerge at different scales of computation. 

        % There are good reasons for the community to search for simple numerical measures of efficiency.  
        % AutoML and Neural Architecture Search (NAS) allow for automatic efficient model design by optimizing jointly for FLOP count and accuracy. Such scores can be customized depending on the researchers' constraints.  For example, hardware-aware approaches directly incorporate latency or energy usage into the NAS search objective \cite{wu2019fbnet, tan2019mnasnet,wang2020hat}. While manual inspection of the learned models shows that NAS often implicitly learns to take advantage of supported parallelism (i.e. learning wider architectures on GPU devices and deeper models on CPU devices) \cite{cai2018proxylessnas,tan2019mnasnet, sandler2018mobilenetv2}, to our knowledge these measures of inference speed are determined wi


\subsection{Hardware and Platform Performance Analysis}
    Efforts to establish common benchmarks leverage reference models and hardware platforms with target latency or accuracy \cite{reddi2020mlperf,janapa2022mlperf, zhou2020hulk}. Although these efforts have led to improvement in end-to-end latency, they often abstract away the underlying frameworks, compilers, backends, and hardware platforms. While general purpose improvements in hardware and software kernels may lead to improvements across all models, it has been argued that solely focusing on performance optimization of a limited set of model architectures and runtimes may lead to overspecialization \cite{hooker2020hardware}.

    Previous analysis of the computational properties of hardware accelerators has largely focused on the training setting in which larger kernels and batch sizes hide framework overhead that emerges in the inference setting \cite{wang2020systematic, zhu2020daydream, zhu2018tbd}. Analyses of overhead in machine learning systems has primarily focused on domain-specific applications, such as reinforcement learning and recommendation systems settings \cite{gleeson2021rl, lin2022building}, where simulation and memory access dominate execution time. These prior efforts are largely restricted to a small set of reference model architectures and have not directly examined the relationship between model and platform in inference across scale.
    

    
% Early deep learning frameworks, such as Caffe \cite{jia2014caffe}, Theano \cite{al2016theano}, and Tensorflow \cite{tensorflow2015-whitepaper}, were developed under an explicit graph and define-and-run paradigm in which computational graphs were built explicitly and then compiled ahead of runtime. In contrast, modern deep learning frameworks, such as PyTorch \cite{paszke2019pytorch} and TensorFlow Eager, are primarily developed under an eager execution, define-by-run paradigm. Eager, in which the computational graph is built by composing operations in the local environment, is favored for its use and debugging. However, this flexibility comes at the cost of additional overhead by executing the computational graph as defined. 

% High-level frameworks abstract away implementation of the underlying tensor operations to linear algebra and neural network packages which implement basic matrix primitives, such as: CUDA and CuDNN on Nvidia GPUs, OneDNN on Intel CPUs, NNPack, OpenBLAS, or Eigen. Depending on input sizes and formats these libraries will select different  algorithms for implementing the matrix operations, such as deciding between FFT, GEMM, winograd for 2D-convolutions. These libraries provide interfaces for execution of tensor operations using vector instruction sets such as AVX and SSE on Intel CPUs, and NEON instruction on ARM CPUs.

    % For ease of development and debugging, high-level frameworks default to an eager-execution approach to graph construction. Just-in-time compilers such as TorchScript and Torch.fx allow for acceleration of computational graphs by fusing redundant operations into a single computation, such as fusion of convolutions and batch norm layers. By completely exiting the high-level framework, models can be accelerated by exporting into inference-specific runtimes such as ONNX. ONNX is a platform agnostic interface for serializing computation graphs into a common format that can be run using a variety of backend execution providers such as: CUDA and TensorRT on Nvidia GPUs, OpenVINO on Intel CPUs, ARM NN on ARM CPUs.  


    


==> sections-es/3_preliminaries.tex <==
    \begin{figure}
         \centering
         \includegraphics[width=0.4\textwidth, trim=0cm 5cm 0cm 0cm]{assets/assets-1/execution.pdf}
         \caption{Profiles where execution is bound by CPU operations (above) and by GPU kernel operations (below). Small compute kernels are common at lower batch sizes and in inference. Boxes with dashed lines represent \textit{framework overhead}. }% as defined in \S\ref{sec:framework-overhead-defn}.}
         \label{fig:framework-boundedness}
         \vspace{-10pt}
    \end{figure}

\section{Framework Overhead}
    Deep learning frameworks often dispatch computation for asynchronous execution on highly parallelized hardware accelerators, as shown in Figure \ref{fig:framework-overhead}. For sufficiently large compute kernels, such as those seen during training, models achieve near maximum GPU utilization as measured by the difference between total execution time and active GPU time \cite{zhu2018tbd}. However, during inference, smaller input sizes frequently lead to suboptimal GPU utilization as the rapid executing kernels do not saturate the fixed cost framework overhead incurred from CPU operations (i.e. kernel launch, computational graph construction, control flow, and device synchronization; See Figure~\ref{fig:framework-boundedness}). 

   \begin{figure}
     \centering
     \includegraphics[width=0.3\textwidth]{assets/assets-1/framework-overhead.pdf}
     \caption{Framework overhead of ResNet-50 in PyTorch for various batch sizes on an RTX-8000. Framework overhead is substantial at low batch sizes but only a small constant at large batch sizes.}
     \label{fig:framework-overhead}
     \vspace{-12pt}
    \end{figure}
    
\label{sec:framework-overhead-defn}
    \begin{figure*}[ht!]
        \centering
        \includegraphics[width=0.95\textwidth]{assets/assets-1/baselines-new.png}
        \vspace{-5pt}
        \caption{Latency vs. batch size for baseline models in FP16 and FP32 on RTX-8000. Framework boundedness exists for all models at small batch sizes where framework overhead dominates runtime regardless of Framework overhead is most prominent in smaller models executed in half precision (FP16) on slower frameworks.}
        \label{fig:baselines}
        \vspace{-5pt}
    \end{figure*}    
    

    When the execution of GPU kernel computation is blocked by CPU framework operations such as kernel dispatches, the model's execution becomes \textit{framework-bound}. In this setting, latency is constant regardless of batch size or number of MACs computed. For settings where latency is dependent on the execution of computational kernels and data movement, we refer to models as being \textit{compute-bound}.


==> sections-es/4-analysis.tex <==
\section{Experimental Setting}    
    \begin{figure}[h!]
        \centering
        \vspace{-4pt}
        \includegraphics[width=0.3\textwidth]{assets/assets-1/framework-optimizations.pdf}
        \vspace{-5pt}
        \caption{Different framework optimizations lead to latency improvements in different regimes. CUDA Graph kernel serialization reduces launch overhead in the framework bound regime, whereas sparse computation reduces latency at larger batch sizes. 
        \label{fig:framework-optimizations}
        \vspace{-8pt}
        }
    \end{figure}    

    
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{assets/assets-1/model-scaling-all.png}
    \label{fig:model-scaling}
    \vspace{-5pt}
    \caption{Comparison of latency for BERT and ResNet variants that scale model \textit{width} and \textit{depth}. Increases in model depth add more framework overhead, whereas increases in model width lead to faster transitions to compute boundedness. ResNet-50 and its Wide ResNet-50 variant are equivalent in latency up to batch size 8 despite having over 3x fewer parameters. }
\end{figure*}    

    
    We evaluate on batch sizes from 1 to 128 and measure average latency of 100 forward passes after 10 warmup passes. GPU core and memory utilization are measured with the PyTorch profiler, Nvidia NSight, and NVIDIA Management Library (NVML), respectively. We randomly generate image data in the 224 x 224 RGB NCHW format, and language data as random embedding sequences of length 128.   



\label{sec:baselines}

\section{Framework Considerations}
    Frameworks adhering to an eager mode of graph construction, such as PyTorch or TensorFlow 2.0, incur overhead from execution inside an interpreted environment given that the time between kernel launches is related to the speed at which kernels are enqueued, which is in turn affected by host-side latency. To mitigate this, inference frameworks such as TorchScript attempt to reduce interpreter overhead and introduce computation graph-level optimizations. 
    Static runtimes can remove interpreter overhead entirely by compiling graphs ahead of time; the ONNX runtime provides further optimizations through graph rewrites that can fuse operators such as GEMMs and convolution layers with subsequent activations or norms. Such fusion operations can reduce memory footprint and result in more efficient kernels, decreasing overall framework overhead.
    
    % Faster frameworks yield less framework overhead
    Unsurprisingly, model latency decreases when performing inference with frameworks and runtimes that support more aggressive optimizations as seen in Figure \ref{fig:baselines}. These increases are especially pronounced at low batch sizes where inference is framework-bound.     
    
    For batch size 1, TorchScript and ONNX provide an average FP16 speed up of 34.16\% and 71.38\% over PyTorch, respectively. As batch sizes increase and models become compute bound, there is substantially less difference in latency across frameworks as the majority of execution time is spent awaiting the completion of kernel execution. 
    
    Although these speedups suggest that inference should always be executed in specialized inference runtimes, static construction of computational graphs may be slower when considering real input data where examples may differ in size, leading to input sparsity.  We consider framework optimizations that utilize kernel serialization and sparse nested tensor operations in Figure \ref{fig:framework-optimizations}. To construct sparse inputs, we simulate samples for sentence processing by generating variable length sequences and padding to the maximum sequence length of 128. Sentences are randomly generated according to the sequence length distribution of the Penn Treebank \cite{taylor2003penn}, with an average length of 20.92 and a standard deviation of 10.18 tokens. We see that CUDA Graphs remove framework overhead at low batch sizes, but the efficiency gains from sparse tensor optimizations lead to latency reductions for larger batch sizes.


\section{Model Design Decisions}
    We select ResNet-50 \cite{he2016deep}, GPT-2 \cite{radford2019language}, BERT-Base \cite{devlin2018bert} as representative architectures of the CNN and transformer architecture paradigms.
    
    Although, the number of FLOPs required for model inference scales with the input batch size we observe that for small inputs latency is constant in Figure~\ref{fig:baselines}. Both ResNet-50 and BERT-Base exhibit framework boundedness for small inputs, where latency is constant regardless of batch size. 
    
    While execution in both single (FP32) and half precision (FP16) is framework bound, slower computation and increased data movement for FP32 execution leads single precision execution to become compute bound at lower batch size. At larger batch sizes, reduced FP16 precision yields expected reductions in latency as compared to FP32.
    

\subsection{Scaling Model Depth \& Width}
    \begin{figure*}[!ht]
        \centering
        \includegraphics[width=0.90\textwidth]{assets/assets-1/model-mobileops.png}
        \vspace{-10pt}
        \caption{Latency of CNN and Transformer models using \textit{efficient variations} of convolution and self-attention operations. All of the variants observe lower latency at large batch sizes, but have worse FLOP utilization. Efficient Transformer variants are slower than BERT at small batch sizes due to the introduction of more layers.}%  See Fig~\ref{fig:bs-efficient-bert} in Appendix~\ref{appx:figs} for batch size comparison in BERT models}. % TODO: Clean up this sentence
        \label{fig:model-mobileops}
    \end{figure*}    
    
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{assets/assets-1/model-pooling.png}
    \vspace{-10pt}
    \caption{Comparison of latency for BERT and Funnel Transformer. Despite using fewer total MAC operations, Funnel Transformer is slower than BERT for inference due to the introduction of additional intermediate pooling layers. }
    \label{fig:model-pooling}
    \end{figure}
    
    \begin{figure*}[!ht]
        \centering
        \includegraphics[width=0.85\textwidth]{assets/assets-1/hardware-new.pdf}
        \caption{Framework overhead becomes increasingly prominently with newer generations of GPU. See Fig~\ref{fig:throughput-gpu} in Appendix~\ref{appx:figs} for an alternative view featuring throughput across generations of GPUs} % TODO: Clean up this sentence
        \vspace{-12pt}
        \label{fig:hardware}
    \end{figure*}
    
     Scaling model hidden dimensions and number of layers are common techniques for exploring tradeoffs between FLOPs and performance.
     For ResNet-50, we examine ResNet-18, 101, and 152 \cite{he2016deep} and Wide ResNet-50 \cite{zagoruyko2016wide}. Similarly, we compare 12-layer BERT-Base against 6-layer DistilBERT \cite{sanh2019distilbert} and variants of BERT with varying depth and width. 

    Increasing number of layers, leads to increases model latency in both the framework- and compute-bound regimes as each added layer operation requires an additional CPU-GPU dispatch, as seen in Figure~\ref{fig:model-scaling}.
    
    Counterintuitively, increases in model width lead to \textit{no increase in latency} at low batch sizes. In this setting, computation is framework bound and total runtime is constant despite the wider operations requiring more floating point operations. However, larger compute kernels causes these wider models to become compute-bound at lower batch sizes. Once compute-bound, latency scales more rapidly with batch size for wide models.
    
\subsection{Downsampling and Hierarchical Pooling}
    Self-attention layers are notoriously expensive as their computational complexity scales quadratically with sequence length. Efficient transformer architectures often attempt to reduce these costs by downsampling the sequence to reduce length and total MACS \cite{dai2020funnel, kitaev2020reformer, wang2020linformer}.   We examine the performance of the Funnel Transformer, which applies average pooling every 4 layers, which attains comparable downstream performance to BERT with $42\%$ fewer total MAC operations through sequence length reduction. 
    
    In Figure~\ref{fig:model-pooling}, we see that Funnel Transformer's reduction in total FLOPs does not translate to increased inference speed. Added pooling layers introduce additional steps to the computation graph, and increase the model's framework overhead. Funnel Transformer is framework bound at a much higher latency than BERT at low batch sizes, and remains slower even at larger batch sizes. 
    % For framework bound models, inclusion of additional layers increases overall latency even if reducing total number of FLOPs.  

    % \begin{figure*}[!ht]
    %     \centering
    %     \includegraphics[width=\textwidth]{assets/assets-1/hardware-new.pdf}
    %     \vspace{-15pt}
    %     \caption{Framework overhead occurs across multiple generations of GPU hardware –- increasingly prominently with newer generations.} % TODO: Clean up this sentence
    %     \label{fig:hardware}
    % \end{figure*}
    

\subsection{Efficient Mobile Operations}
    Low-FLOP operations are commonly used as substitutes for dense convolution and linear operations in edge settings. 
    In Figure~\ref{fig:model-mobileops}, we examine models utilizing grouped convolutions: SqueezeNet \cite{iandola2016squeezenet} and SqueezeBERT \cite{iandola2020squeezebert}; inverted residual bottlenecks MobileNet \cite{sandler2018mobilenetv2}, EfficientNet \cite{tan2019efficientnet}, MNasNet \cite{tan2019mnasnet}, and MobileBERT \cite{sun2020mobilebert}.
    
    While these operations reduce the number of FLOPs required for execution, they exhibit worse per-FLOP latency and poor memory utilization as compared to baseline models. In fact, for the case of the transformer architectures, both grouped convolutions and inverted bottleneck operations in these efficient architectures lead to worse latency than baselines. Similar to pooling operations, these operations introduces substantial framework overhead that slows down execution for low batch sizes. 
    % However, at large batch sizes, reduction in FLOPs yields empirical wall-clock gains over a BERT baseline. 
    % Additionally, these operations can suffer in deployment settings where component depthwise and pointwise convolutions may have limited hardware and framework support.  



    
    % or limited support for component operations. Inference runtimes often support only a subset of the available operations in more flexible eager frameworks designed for research and prototyping, and thus require CPU fallback operations. 
    % For example, FNet is a BERT variant which replaces self attention layers with Fast Fourier Transform (FFT) operations. Although FFTs are deterministic operations with good hardware support, they are not in the ONNX opset. In this case, FNet executed with eager PyTorch is still XX ms faster than BERT despite using a less optimized framework. 
    % Additionally, custom frameworks can often lag the research community and lack support from the most recent libraries implementing matrix primitives. For example, PyTorch is released with CUDA 11.8 at the time of writing. By comparison, ONNX Runtime only supports CUDA 11.6. Each framework can differ in terms of the quality and choice of the kernels in the backend libraries they utilize for matrix operations, and this can also impact the translation from FLOPs to latency. %  We observe that while the low-batch latency with ONNX is substantially faster than PyTorch and TorchScript, the ONNX Runtime is slower at large compute bound batch sizes which we attribute to it's older version of CUDA which may be leveraging slower compute kernels.  % Cite 

\section{Hardware Considerations}
    In Figure~\ref{fig:hardware}, we observe that framework-bound inference emerges across multiple generations of consumer, workstation, and datacenter Nvidia GPUs. As the speed of the accelerator increases, the relative execution speed of the compute kernels decreases while the total framework overhead due to CPU kernel dispatch operations remains constant. 
    % We observe that GPUs that lack Tensor Core support for half precision operations, such as the 1080Ti, are notably slower and less framework-bound than newer GPUs. Conversely, execution on faster GPUs, such as the RTX 3090 and the A100, remains framework bound until larger batch sizes.
    These observations indicate that framework bounds on model execution will continue to worsen as hardware improves unless commensurate improvements are made to deep learning frameworks.
    % For example, BERT-Base is not framework bound for older 1080Ti GPUs but is 
    
    % The largest contributor to framework overhead is to CPU dispatch operations. As a result, the fixed latency for framework-bound models is a product of the entire system's configuration, dependent on hardware specifications such as the CPU and memory speeds. In contrast, the latency of compute-bound models is mainly determined by the selected kernels and their supported FLOPs per second by the GPU, with faster GPUs yielding faster execution.


% Examination of the runtime profiles shows low GPU utilization of these models for inputs with small batch size; reported in Table \ref{tab:gpu-util}. Until the runtime of the GPU compute kernels is sufficiently large, the overall model's latency is constant blocked by CPU operations managing the computational graph and dispatching kernel launches. Qualitatively, this is observed in runtime profiles in figures \ref{fig:pytorch-profile}, \ref{fig:jit-profile}, \ref{fig:ONNX-profile}. 

% Analysis
% GPU Performance Analysis
% 1. Framework and memory overhead leads to low GPU utilization at small input sizes
% 	- Results in constant time execution
% 	- Layers are a reasonable proxy in the bounded region
% 	- FLOPs are a reasonable proxy in the compute bound region
% 	- Caveats: 
% 		- Graph overhead is dependent on framework, CPU, architecture
%		- FLOP are not entirely predictive of latency; depends on memory locality of operations, type of operation, algorithm, hardware

 
  % 1. Latency vs MACs
  %		0. Latency vs MACs: Doesn't work
  %		a. Find memory bound region: Latency vs Average MACs per layer
  %			- Separate based on highest FLOP layer type
  %			- Exceptions and Other Cases: 
  % 			- Branched Models, 
  % 			- Models with mixed operation types: Efficient Net V2, SqueezeNet, ShuffleNet
  %		b. Plot latency vs total MACs the compute bound region
  % 2. Find latency in the memory bound region
  % 	a. Model Depth
% Comparison Across GPU Architectures
% 	1. NVidia Architecture Generations
%	2. Edge vs Server: CPU and GPU
% Effects of Hardware and Platform Optimization
% 	0. Vector Extensions on CPU:
% 	1. Mixed Precision: Super linear increase in compute
%	2. Tensor Core Utilization: Increases in speeds but model performance is still generally bounded by CUDA core speed
%	3. Model Serialization and JiT: ONNX and Torchscript
    

% In training and at large input sizes, framework overhead is negligible. Hardware utilization is low at small input sizes, which increases the impact of framework overhead on total runtime. For small batch inference settings, eager execution frameworks limit computational efficiency. Actual framework overhead is variable across a number of factors including framework implementation and CPU. 


% \begin{figure*}[!ht] 
%      \centering
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/resnet-bs1.png}
% 		 \caption{ResNet-50 Profile at Batch Size 1 with standard PyTorch.}
%          \label{fig:pytorch-profile}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/jit-resnet-bs1.png}
%         i \caption{ResNet-50 Profile at Batch Size 1 with PyTorch TorchScript.}
%          \label{fig:jit-profile}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/ONNX-resnet-bs1.png}
%          \caption{ResNet-50 Profile at Batch Size 1 in the ONNX Runtime. }
%          \label{fig:ONNX-profile}
%      \end{subfigure}
%     \caption{PyTorch and TorchScript exhibit low GPU utilization for batch size 1 due to blocking on CPU kernel dispatches. ONNX Runtime with the CUDA backend observes high GPU utilization with minimal gaps between kernel execution.}
%     \label{fig:profiles}
% \end{figure*}






% \subsection{Comparison of Hardware Platforms}
% We observe similar patterns of framework bound behavior across multiple generations of Nvidia GPU architectures. Noteworthy, model latency on the Jetson Nano is not obviously framework bound when utilizing an ONNX runtime. This suggests that edge devices achieve reasonably high hardware utilization and low framework overhead due to the limitations of their speed of computation.



% \textbf{Latency in Compute Bounded Regimes}
% After the individual layers have saturated, latency begins to increase linearly according to FLOPs. In this regime, FLOPs are a strong predictor of latency with a Pearson rank correlation of 0.95.

% In figure \ref{fig:GPU_Utilization}, we examine the inference profile of ResNet-50 on an RTX-8000. We observe that for single-example inference there is low GPU utilization as computation is blocked by CPU-operations. Even on efficient models designed for edge devices, such as MobileBert on the Jetson Nano, GPUs fail to achieve high utilization and are blocked by kernel launches.




% TODO: Add figures for BERT (Batch Size and Sequence Length), Res-Net, Inception

% Performance Analysis
% 1. Each operation has a different amount of peak FLOP utilization per platform -- See FLOP utilization heat maps
% 2. Each operation saturates (memory to compute bounds) at a different point -- See roofline
% 3. Operation X Hardware Saturation Point is determined by number of MACs that corresponds to ???
% 4. Memory vs Compute Bound Regime can be determined by:
	% a. Identifying type of operation with the highest number of FLOPs
    % b. 
    % Exceptions: 
% 5. Latency can be determined by:
	% a. Memory Bound Region: Latency is constant regardless of input size 
    
% Model Design Recommendations
% 4. 

% All Parallel Core Architectures Follow Roofline Behaviors
	% Previous work has shown this for single example inference and individual operations
    % Unlike previous work which finds individual operations are memory bound, in the inference setting the model overall is compute bound for most standard input sizes
    % 

% Not all Operations are the same
% While the computational graph creates a more complex transition between memory and compute-boundedness we can approximate it via average MACs in the operationally densest layers (i.e. Conv2D and linear). 
	% Each model observes a different trajectory in both regimes due to differing proportions of operations and layer, framework overhead
    
% Max utilization can be achieved by ensuring input size >= compute boundedness
% Latency is determined by 
% with an \textit{r}-squared value of 0.87 and RMSE of TODO. Similarly, on the Raspberry Pi-4B . 

    
    
% \subsubsection{FLOPS Utilization}
% \label{section:flops-util}
% % TODO : GPU Operations Heatmap
% \begin{figure}
% 	% \includesvg{assets/rtx-floputil.svg}
%     \caption{TODO: FLOPS Utilization RTX-8000}
%     \label{fig:rtx-roofline}
% \end{figure}

% In this section, we investigate the FLOPs utilization at the layer level for fully-connected linear layers, standard 2D convolutions, and factorized inverted bottleneck convolutions. 

% In figure HEAT-MAP, we observe that both 2D-convolution layers and linear layers approach a similar bound on FLOPS utilization. By comparison, the MB-Convolution observes a much lower peak FLOPS utilization due to low arithmetic intensity of its component depthwise-convolution \cite{gholami2018squeezenext}.

% \subsubsection{Memory Bandwidth and Roofline Analysis}
% \label{section:roofline}
% % FIGURE: GPU Roofline Plots
% \begin{figure}
% 	\includesvg[width = 240pt]{assets/rtx-roofline.svg}
%     \caption{Roofline Plot for RTX-8000}
%     \label{fig:rtx-roofline}
% \end{figure}

% In Figure \ref{fig:rtx-roofline}, we show hierarchical roofline plots computed for the RTX-8000. There is a sizable gap between the peak floating point operations per second (FLOPS) and the observed computational intensity of the reported models. 

% We observe that models approach differing peak FLOPS per second. However they approach similar compute bounds on maximum arithmetic intensity as measured in FLOPS.   

       


%  \subsection{CPU Performance Analysis}
% 	Without parallel-core support, model inference is compute bound at all input sizes on CPU-based platforms. In this setting, total latency L and throughput can easily be approximated with a theoretical FLOPs proxy:
%     % $$ \text{Latency} = \frac{\text{Threads} \times \text{Clock Speed}}{\text{SIMD Parallelism}}$$
%     For instance, on Intel Xeon with AVX-2 extensions, supporting 8 concurrent SIMD operations. This baseline model matches ground truth latency recision reduces the memory traffic of operations.
    
    
%     \subsubsection{Just-in-Time Compilation}
%     ONNX and Torchscript

%     % \subsection{Framework Choice}


==> sections-es/5-discussion.tex <==
\section{Discussion}

\paragraph{Computational graph optimizations and compilation improve latency.}
Removal of host language dependencies and graph optimizations provides substantial speedups over eager frameworks for inference at low batch sizes. However, feature completeness for operators and control flow varies across graph optimizers and compilers. For example, the FNet architecture \cite{lee2021fnet} relies on FFTs as a swap-in for self-attention. Currently, FFT operations are not currently supported by ONNX or TorchScript.
% and to our knowledge, no JIT compilers support graph rewrites that add FFTs.
As expected, FNet executed in PyTorch outperforms BERT executed in ONNX RT despite less framework overhead -- with a 10.31\% speedup at batch size 1. 
% For improvements in research to translate to deployment, additional investment can be directed towards support for complex control flow and operators in inference runtimes. 

\paragraph{Dynamic computational graphs can be faster for input sentences with variable lengths.} Dynamic computational graphs can leverage input sparsity to reduce latency when processing variable length text. For example, PyTorch with sparse tensor optimizations reduces the latency of BERT-Base using static CUDA graphs by 80.56\%  at batch size 128 when processing sparse inputs. 

\paragraph{At large input sizes, framework overhead from graph operations is negligible.}
For batch sizes larger than 16, we find there is minimal latency difference across models, inference runtimes, and frameworks. In the compute-bound regime, number of FLOPs is still a poor latency predictor due to variable execution time for different operations. For example, mobile architectures that depend on inverted-residual layers are memory inefficient and are much slower per-FLOP than standard convolution and GEMM layers.

\paragraph{For framework-bound models, model depth is a reasonable proxy for latency.}
Number of floating point operations is a poor indicator of latency in a framework-bound setting, as total runtime is generally constant and tied to framework overheads and the size of the computational graph. In framework-bound models, the size of the computational graph is related to model depth.

\paragraph{Estimations of latency for models deployed in production settings must account for their target framework and hardware platform.}
Model development frequently occurs using eager execution research frameworks. However, deployment often occurs in inference runtimes and on mobile devices or specialized hardware. This misalignment can mislead the development of ``efficient'' models and result in claimed gains that do not translate to real-world deployment settings. As such, researchers should be clear in specifying the setting of their ``efficiency" gains, such as the target frameworks and hardware platform, when developing new methods. For example, techniques such as hardware-aware neural architecture search which leverage direct latency measures must also control for framework choices to account for this mismatch.


% \paragraph{Throughput and input size can be increased at minimal cost for framework-bound models.}
% For a given model, latency is constant regardless of batch size until compute kernels saturate and exceed CPU launch costs. If computation is bottlenecked by framework overhead, the batch size or input size can be increased without increases in overall runtime. In practice, this can lead to the processing of larger batch sizes and sequence lengths at no additional latency cost until kernel operations saturate framework overhead. 

\begin{table}[!t]
    \scriptsize
    \centering
    \begin{tabular}{@{}rrrrrr@{}} \toprule
    \textbf{SA Dim} & \textbf{FC Dim} & \textbf{Batch} & \textbf{Seq Len} & \textbf{Latency} & \textbf{Throughput} \\ \midrule
    \phantom{0}768 & 3072      & 1           & 128      & 0.0136    & 0.0136   \\ 
    \phantom{0}768 & 3072      & 4           & 128      & 0.0134    & 0.0034   \\ 
    \phantom{0}768 & 3072      & 1           & 512      & 0.0134    & 0.0134   \\ 
    1536           & 6144      & 1           & 128      & 0.0134    & 0.0134   \\ 
    \bottomrule
    \end{tabular}
    \caption{Latency of BERT PyTorch models on RTX-8000. Scaling along batch sizes and model width shows no increase in latency.}
    \label{tab:scaling-bert}
    \vspace{-16pt}
\end{table}

% \paragraph{Model width can be increased at no cost for framework-bound models.}
% For a given batch size, individual layers of a framework bound model can be made wider by increasing hidden dimension or filter size without impacting latency. Wider models are known to exhibit better task performance due to increased parameter count and expressivity \cite{zagoruyko2016wide}.

% Model designers can leverage wider architectures with their target inference framework and hardware setting in mind to achieve higher utilization. For example, models processing few examples during inference can leverage wider layers to avoid CPU framework bottlenecks. See Table~\ref{tab:scaling-bert}.

\paragraph{Using higher-performing hardware does not necessarily improve end-to-end performance.}
Framework overhead limits the impact of improved hardware as it limits utilization. This trend will continue as ML-specific hardware advances without efforts to address software bottlenecks. For example, single-example inference with both BERT is slower using an A100 than using a V100 GPU despite a 2.75x increase in peak computational throughput.



\section{Conclusions }
In this work, we conduct an study of neural networks from the CNN and transformer architecture paradigms across a variety of software and hardware platforms. We show that inference performed with these large neural networks, which was previously assumed to be compute bounded, is in fact limited by overhead incurred by deep learning frameworks -- a phenomena we refer to as the \textit{framework tax}. In particular in the inference setting when compute kernels can be executed quickly, we show that existing methods of designing efficient model architectures are in fact limited by limitations in framework design.
% In particular, we examine execution bottlenecks that emerge due to kernel dispatch operations commonly used by accelerator-enabled deep learning frameworks as they introduce the largest bottleneck to latency. 
% In Appendix \ref{appx:cg}, we see that while fully-compiled CUDA graph latency largely addresses this source of framework overhead, CUDA graphs still suffer from low GPU utilization at small input sizes. 
% In future work, we intend to study other sources of framework overhead and additional causes of misalignment between model architectures and hardware platforms.

% While wider transformer architectures (e.g. BERT-Base) exhibit less boundedness behaviors than narrower, deeper CNNs (e.g. ResNet-50), we show that all models exhibit framework boundedness.  Additionally, we observe that these inefficiencies are becoming more apparent as hardware accelerator speeds increase. 


% \begin{table}
% \scriptsize
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \textbf{Self-Attn Dim} & \textbf{FC Dim} & \textbf{Batch} & \textbf{SeqLen} & \textbf{Latency} & \textbf{Throughput} \\ \toprule
% \phantom{0}768 & 3072      & 1           & 128      & 0.0136    & 0.0136   \\ 
% \phantom{0}768 & 3072      & 4           & 128      & 0.0134    & 0.0034   \\ 
% \phantom{0}768 & 3072      & 1           & 512      & 0.0134    & 0.0134   \\ 
% 1536           & 6144      & 1           & 128      & 0.0134    & 0.0134   \\ 
% \bottomrule
% \end{tabular}
% \caption{Latency of BERT PyTorch models on RTX-8000. Scaling along batch sizes and model width shows no increase in latency.}
% \vspace{-15pt}
% \label{tab:scaling-bert}
% \end{table}

% \textbf{Throughput and input size can be increased at no cost for framework-bound models.}
% For a given model, latency is constant regardless of batch size until compute kernels saturate and exceed CPU launch costs. If computation for a particular input size is bottlenecked by framework overhead, the batch size or input size can be increased without increases in overall runtime. In practice, this can lead to the processing of larger batch sizes, sequence lengths, or higher image resolutions at no additional latency cost until kernel operations saturate framework overhead. See Table~\ref{tab:scaling-bert}.

% \textbf{Model width can be increased at no cost for framework-bound models.}
% For a given batch size, individual layers of a framework bound can be made wider by increasing hidden dimension or filter size without increases in latency. Wider models are known to exhibit better task performance due to increased parameter count and expressivity \cite{zagoruyko2016wide}.

% Model designers can leverage wider architectures with their target inference framework and hardware setting in mind to achieve higher utilization. For example, models processing few examples during inference can leverage wider layers to avoid CPU framework bottlenecks. See Table~\ref{tab:scaling-bert}.

==> sections-es/appx-cudagraph.tex <==
\section{Results Using Precompiled CUDA Graphs}
\label{appx:cg}
CUDA Graphs are an optimization that enable compilation and serialization of multiple CUDA kernels and remove the need for repeated kernel dispatch calls. As such they can significantly reduce framework overhead, however they still observe low hardware utilization. 

\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{lllll}
\textbf{Batch Size} & \textbf{Latency (ms)} & \textbf{SMs Active} & \textbf{Warp Occupancy} & \textbf{Memory Throughput (R | W )} \\ \toprule
1                   & 2.81                  & 57.0\%              & 9.2\%                   & 5.3\% | 2.3\%                       \\
2                   & 3.07                  & 63.4\%              & 17.6\%                  & 13\% | 8\%                          \\
4                   & 3.95                  & 64.4\%              & 25.6\%                  & 9.5\% | 9.2\%                       \\
8                   & 6.02                  & 73.4\%              & 32.4\%                  & 13.0\% | 13.1\%                     \\
16                  & 10.84                 & 78.1\%              & 39.6\%                  & 16.5\% | 15.3\%                     \\
32                  & 20.65                 & 82.8\%              & 42.4\%                  & 21.7\% | 16.5\%                     \\
64                  & 35.77                 & 93.5\%              & 47.9\%                  & 24.9\%| 19.1\%                     \\ \bottomrule
\end{tabular}
\caption{GPU Utilization of BERT-Base executed in PyTorch with CUDA Graphs on an RTX-8000.}
\end{table}

\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{llllll}
\textbf{Framework}            & \textbf{Compilation} & \textbf{Kernel Serialization} & \textbf{Latency} & \textbf{SMs Active} & \textbf{Warp Occupancy} \\ \toprule
PyTorch                       & Eager                & None                          & 10.54 ms         & 2.6\%               & 0.9\%                                  \\
PyTorch with TorchScript      & Just-in-Time         & None                          & 6.14 ms          & 18.5\%              & 3.0\%                                       \\
PyTorch with CUDA Graphs      & Eager                & Yes                           & 2.82 ms          & 57\%                & 9.2\%                    \\
ONNX RT                  & Ahead-of-Time        & None                          & 2.56 ms          & 22.3\%              &   9.5\%                       \\
ONNX RT with CUDA Graphs & Ahead-of-Time        & Yes                           & 2.11 ms          & 59\%                & 20.3\%    \\                          \bottomrule
\end{tabular}
\caption{Comparison of SM Activity Across Frameworks for BERT-Base at batch size 1. CUDA Graphs enable higher GPU utilization but still observe low levels of SM activity and warp occupancy.}
\end{table}

==> sections-es/appx-speech.tex <==
\section{Additional Experiments: Speech}
\label{appx:speech}
 In Figure \ref{fig:model-speech}, we examine the behavior of the WavLM \cite{chen2022wavlm} model which consists of a CNN encoder followed by transformer encoder layers. Audio inputs are simulated as 2 second sequences sampled at 16 kHz to create 32,000-dimensional floating point inputs.  As with transformers and CNNS,  we observe that WavLM exhibits framework bound behavior but quickly transitions to being compute-bound due to the large audio sequence lengths in Figure \ref{fig:model-speech},
 

 \begin{figure}[!h]
    \centering
    \includegraphics[width=0.4\textwidth]{assets/assets-1/speech.pdf}
    \caption{
    Transformer-based speech models exhibit framework boundedness but transition to compute-bound at small batch sizes due to long sequence lengths.
    % See Fig~\ref{fig:bs-efficient-bert} in Appendix~\ref{appx:figs} for batch size comparison in BERT models
    } % TODO: Clean up this sentence
    \label{fig:model-speech}
    \vspace{-12pt}
\end{figure}    


==> sections/0_abstract.tex <==
\begin{abstract}
Increased focus on the efficiency of machine learning systems has led to rapid improvements in hardware accelerator performance and model efficiency. However,  the resulting increases in computational throughput and reductions in floating point operations have not directly translated to improvements in wall-clock inference latency.  We demonstrate that these discrepancies can be largely attributed to bottlenecks introduced by deep learning frameworks. We denote this phenomena as the \textit{framework tax}, and observe that the disparity is growing as hardware speed increases over time. In this work, we examine this phenomena through a series of case studies analyzing the effects of model design decisions, framework paradigms, and hardware platforms on total model latency.  Based on our findings, we provide actionable recommendations to researchers and practitioners aimed at narrowing the gap between efficient ML model research and practice.

% Recent algorithmic, hardware, and software-based advances in machine learning (ML) have enabled dramatic improvements in accuracy across tasks in vision and language, with modern approaches requiring significant computational resources. These improvements have driven a widespread interest in deploying models at scale, with inference latency emerging as a principal criterion for real-world deployment. Despite their widespread use, proxies for latency such as multiply-accumulate (MAC) or floating-point operations per-second (FLOPS) fail to take into account important hardware and software-related factors. In this work, we conduct an extensive empirical study of these and other metrics and analyze their failures to predict latency and throughput
% In response we introduce a new metric, known as \textit{framework overhead}, that measures hardware-software model efficiency and utilization.
%We provide guidance for efficient model design.   
\end{abstract}

% rewrite notes from 1/25/23 meeting:
% 1. Despite rapidly growing research community/results in ML efficiency (bonus points for intro: quickly get some numbers on number of papers published w/ e.g. efficient/efficiency in title in ICML, ICLR and NeurIPS over past couple of years), these improvements are slower to translate into practice/deployment
% 2. This is due to a mismatch in terms of metrics and frameworks used -- flops don't correspond to metrics used in deployment (latency)
% 3. In this work we demonstrate this discrepancy through a series of case studies ... (describe extent of experimental setup a bit) and provide actionable recommendations to researchers and practitioners based on our findings

% Deep learning is a compute-intensive application that often requires billions of floating point operations to compute inference for a single example. Fortunately, GPUs support similarly massive parallelism that allows for substantial speedups of model execution. In this work, we evaluate common real-world pretrained models from natural language processing and computer vision across multiple generations of commodity GPU hardware and edge settings to provide an analysis of factors that affect the model latency and provide guidance for model design and optimizations. One such finding is that in inference, common eager execution frameworks incur substantial overhead from launching kernel operations leading to low GPU utilization, implying that model width and batch size can be scaled at no cost to latency for models bound by such framework overhead.

==> sections/1_intro.tex <==
\section{Introduction} 
    % Model design has been accelerated by hardware and platform advances
    % The development of machine learning frameworks such as PyTorch \cite{paszke2019pytorch} and TensorFlow \cite{tensorflow2015-whitepaper} has greatly reduced the barrier to entry for deep learning research. At the same time, advances in specialized hardware accelerators, has led to significant performance improvements in the execution of deep learning workloads. Combined, these innovations in hardware and software have enabled rapid progress in the fields of machine learning (ML) and artificial intelligence (AI), resulting in notable achievements such as human-level performance on popular benchmarks in computer vision and natural language processing.

    % Inference efficiency is important, understudied; 
    % Neural networks models have achieved human-level performance in popular natural language processing and computer vision benchmarks. These advances have been facilitated by the development of machine learning frameworks, which have reduced the barrier to entry for deep learning research, and by the development of hardware accelerators.led 

    
     Machine learning efficiency is especially important in inference settings when models are used repeatedly and at scale, in contrast to training which poses a single upfront computational cost. For example, Meta reports that inference workloads make up 70\% of their AI power consumption, with the remaining 30\% due to training and development \citep{wu2022sustainable}, while Google attributes 60\% of their ML energy consumption to inference \citep{patterson2022carbon}. Inference is also estimated to make up 80 to 90\% of ML cloud computing demand \cite{barr2019amazon, leopold2019aws}.  In particular, metrics of model speed such as latency and throughput are essential for inference workloads that are subject to real wall-clock time constraints such as in autonomous driving and automated speech recognition \cite{reddi2020mlperf}.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.4\textwidth]{assets/assets-1/figure1-rev1.png}
        \vspace{-5pt}
        \caption{Latency as a function of a model’s multiply accumulate operations (MACs) on an NVIDIA 2080ti GPU. Expected relationships do not hold; model complexity and hardware capabilities fail to predict latency due to framework-boundedness.}
        \label{fig:fig1}
        \vspace{-15pt}
    \end{figure}    

    These concerns have motivated research in both computer systems and machine learning, leading to the development of faster hardware accelerators and more efficient neural network model architectures. In the past five years alone, the number of papers that mention the terms \textit{efficient} or \textit{efficiency} in top machine learning venues has grown by over 250\%. This work has spurred innovations in efficient neural network architecture design aimed at reducing the amount of computation required to achieve a result, often measured as the number of trainable model parameters, floating point or multiply-accumulate operations (MACs) \cite{tan2019efficientnet, dai2020funnel, sun2020mobilebert}. 
    
    Over the same period, the GPU hardware accelerators that power many modern machine learning applications have seen similar performance improvements with the number of floating point operations per second (FLOPS) growing by over 175\%. Despite this progress, the supposed gains offered by faster hardware and more efficient models are often not realized in deployment settings, where model speed has not improved as seen in Figure~\ref{fig:fig1}.

    We find that this misalignment is primarily attributable to overhead incurred by the machine learning frameworks used to implement and execute neural network models in practice. 
    In the past, the runtime of large neural networks in computer vision and natural language processing has been assumed to be compute-bounded by the computation of expensive tensor operations \cite{li2020xsp}.  However, as the speed of hardware increases, the overhead introduced by the deep learning frameworks used to implement and deploy these models is no longer negligible and imposes bottlenecks on overall model execution. 
    
    % Add a transition from last paragraph
    In this work, we conduct a systematic investigation in which we find that improvements to machine learning model architectures and hardware have not translated into reductions in overall inference latency due to overhead introduced by deep learning frameworks. We refer to this phenomena as the \textit{framework tax}, and show that it exists across all deep learning framework paradigms (e.g. eager execution, just-in-time, and ahead-of-time compilation). Due to the fixed framework overhead that dominates the execution time at small batch sizes, proxy measurements of model efficiency used to motivate efficient model design, such as MACs and parameter count, are not predictive of inference latency. Furthermore, we note that existing efforts to improve model efficiency by designing faster GPU kernels do not reduce latency, when total execution is still bound by fixed framework overhead. 
    Moreover, as hardware performance increases and reduces the time for computational graph execution, machine learning systems are \textit{increasingly} framework-bound at larger batch sizes. 
    
    %  We show that this trend not only holds across deep learning framework paradigms (e.g. eager execution, just-in-time, and ahead-of-time compilation), but also becomes \textit{more prominent} as hardware performance increases; as computational graph execution times are reduced, machine learning systems are increasingly framework-bound at larger batch sizes. 
    
    An exhaustive comparison of the rapidly growing space of models and hardware platforms is out of scope, so we instead identify the most popular model components, inference environments, and hardware accelerators for testing (i.e. isolating the cases most likely to mislead a practitioner). More precisely, we analyze the performance of convolutional neural networks (CNNs) and transformer models in eager execution PyTorch, just-in-time compiled TorchScript, and an ahead-of-time compiled ONNX runtime using a CUDA execution provider. We perform our study across seven different GPUs from the Pascal, Turing, and Ampere Nvidia GPU microarchitectures.

    Based on our findings, we provide a series of recommendations for ML researchers and practitioners presented through a collection of case studies.
    Among these, we argue for increased usage of inference runtimes in small batch size settings as they observe substantially less framework overhead. Alternatively, when using eager execution-based frameworks for inference, we recommend increasing model width or batch size to take advantage of increased model capacity. 
    For example, hidden dimensions in self-attention and fully connected layers can be doubled to increase model capacity without affecting latency, implying that model designers have an extra degree of freedom often overlooked when designing around parameters or FLOPs.
    We hope that our analysis and recommendations will help bridge the gap between efficient ML research and practice.
    
    % Alternatively, we recommend increasing model width or batch size for inference with eager execution-based frameworks that have larger per-layer overhead to take advantage of increased model capacity at no cost to latency. 
    
     % We confirm existing observations that hardware and implementation support result in differing peak rates of computation for different arithmetic operations \cite{cai2018proxylessnas, sandler2018mobilenetv2}. As seen in Figure~\ref{fig:MacsLatency}, we observe that as hardware speed increases model latency is no longer a function of the amount of computation being performed.
     
    % However, these commonly used efficiency cost indicators often correlate poorly with direct measurements of model performance, as seen in Figure~\ref{fig:MacsLatency} -- observing that FLOPs is a poor predictor of latency. These measures are intrinsic to a model's architecture and are oblivious to the supporting framework and hardware. As a result, they ignore infrastructure details that are important in predicting a model's actual performance when deployed in practice, such as the management of kernel launches, the sequential structure of the computational graph, and the supported parallelism of underlying hardware. Optimization of model architecture design towards these metrics potentially misleads the ML community into designing purportedly efficient models that fail to meet latency requirements when deployed in practice and generalize poorly to other hardware.

    % Software advances have been developed independently of hardware leading to mismatch in utilization
    % In this work, we systematically evaluate the impact of model architecture, framework and hardware platform on model latency in the inference setting. We examine how different approaches to efficient model design impact wall-clock latency. We examine how different framework paradigms (e.g. eager execution, just-in-time and ahead-of-time compilation) can be used to accelerate model execution. We observe that the software frameworks used to implement and execute neural networks introduce bottlenecks to inference latency, and introduce the new metric of \textbf{framework overhead} to quantify this property.



% (1) peak rate of computation is dependent on the type of arithmetic operation being performed, (2) density of arithmetic operations is inconsistent across layers, (3) sequential dependencies in a neural network model's computational graph limit the degree to which hardware parallelism can be exploited. These properties lead each neural network architecture to exhibit different levels of compute and memory boundedness for a given hardware. Motivated by these insights, we develop a systematic method for evaluating the impact of model architecture, deep learning framework, and hardware platform on model latency. 

% Using these insights, we discuss how alignment of parallelism between model architecture and hardware, software platforms can be best leveraged to increase throughput and hardware utilization. We discuss model design implications and pareto-optimal scaling of model hyperparameters such as layer width.

% As seen in Figure \ref{fig:MacsLatency}, we verify existing results that while number of MACs are a reasonable proxy for speed on CPU-based devices, it is poor indicator of model speed on parallel core architectures. In section \ref{section:flops-util}, we show that this misalignment can be attributed to two main factors: different operations having differing FLOP utilization, model architecture imposing dependency bottlenecks that limit parallel computation. In section \ref{section:roofline}, we show that all models are in fact both memory and compute bound depending on the size of input and number of per-layer FLOPs. In section \ref{section:latency}, we show that the factors that effect model speed in each regime and propose a more comprehensive model for latency estimation. 


% High-Level Goal: Fast and Performant Models
%	- High expressivity: Deeper models, and more parameters per layer
% 	- Low Latency, Throughput: Cheap or Fewer operations 
% 1. Parallellism lets us beat FLOPs as a metric; 
% 	- Not all FLOPs are the same
% 		- Some operations are more expensive
%		- Overhead and underutilized parallelism negates the cost of increased FLOPs 
% 2. Inference compute landscape is complicated by the structure of the underlying hardware
% 	- Memory Bound vs Compute Bound
% 3. 

% Meanwhile, efforts to benchmark hardware and software platforms target fixed  reference models and workloads, leading to the development of custom hardware platforms and compute kernels.  
% Fixed is not entirely true

% There exists a disconnect between the 
% Guidance:
%     - Frameworks: Reduction in the overhead; Speedups are obtainable through layer fusion and serialization

% Motivation: Real-world throughput and latency is an important dquality of neural network models. 
%     - Deployment of edge and specific use-case modeling is a case for hardware-software codesign; i.e. Understand how well a model architecture leverages its target hardware platform
%     - Neural Architecture Search learns these properties implicitly but inefficiently 
%     - Continuous Latency Constraints are not representative of underlying system behavior

% Research Questions
% 0. Question: What determines the actual latency of a model
% 1. Question: How does one determine the overhead of a model? Why do models differ in their roofline heights?
%     - Hardware Support: 
%         - Computation parallelism
%     - Model and Platform properties:
%         - Easy Cases:
%             1. Computational Complexity is Constant throughout the model and it saturates together
%             2. Computational Complexity is Dominated by a Single Operation 
%         - Hard Case: 
%             1. Multiple and Staggered Bottlenecks -- Majority of Computation is not in the "most complex" operation, i.e. DenseNet
%             2. Average latency 
% 2. Question: When does a particular model architecture saturate its compute resources?
%     A. Compute boundedness is dependent on the saturation of operations
%         A1. Bottlenecks for a single model architecture is primarily dependent on operation selection and support

% 3. Can we apply a transformation or model f(hardware, architecture/operation) to determine relatively when operations saturate?
%     - Per operation: 

% Proposals:
% 1. Parallelized Latency is non-linear piecewise:
%     - Memory, Overhead Bound Regime 
%         - Operation Setup + Teardown + Model, Layer Overhead >> Computational Complexity Time
%     - Operation Saturation Regime
%         - Saturation roughly occurs on a per-layer basis
%             0. Find Saturation Points of Conv2D, MBConv, Linear, BatchNorm2D, LayerNorm
%             1. Equivalence of Different Operations to GEMMs
%         - Proposed Experiment and Case Studies:
%             0. Examine Saturation of Homogeneous Models (ResNet and ViT)
%             1. Examine Saturation of Funnel Transformer
%             2. Examine Saturation of Multimodule Models (Inception Net)
%         - Memory Bandwidth Complexity Increases alongside computational complexity (i.e. Roofline max)
%     - Full Computational Bound, Saturation:
%         - Caveats: CPU Fallback on Large Batch Size
% 2. Determining Saturation on a Platform:
%     - Precision 
% 3. Conclusions: 
%     - Optimal hardware-software single example throughput should optimize under the saturation constraint instead of FLOPs 

% Orthogonal Work
%  - JiT Compilation: Computational 
%  - Mixed Precision: 


% Contributions
% 1. Examination of model architecture and hardware as factors on computational bottleneck
%     - Effects of 
%     - Accross Architecture Paradigms: Transformers and CNNs
% 2. Methodology for determining bottlenecks and Target Latency for NAS results
%     - Reduction in Search Space 
% 3. Not a proxy or hand tuned measure

% Model Development Guidance:
% 1. Any operation in the overhead constrained regime is pareto suboptimal
% 2. 

% Additional Experiments: 



% 2. Decomposing the separations:
%     - Well implemented common operations: MM, Conv2D
%     - Overhead: Python Runtime, Kernel Launches
%     - Poorly Parallelized Implementations: 


% General roofline analysis for neural networks fails because models vary across their archit ectures and their constituent operations. 

% Additionally, the focus on operation throughput does not account for the often more important sample level throughput.


==> sections/2_relatedwork.tex <==
\section{Related Work}

\subsection{Efficiency Metrics \& Efficient Model Design}
        To measure model efficiency, metrics intrinsic to the model architecture are often reported such as the number of trainable parameters, number of floating point (FLOPs) or multiply-accumulate (MACs) operations. Number of trainable parameters is a frequently reported metric as a proxy for memory usage.  However, parameter count is often not predictive of model speed \cite{zhou2020hulk} and techniques such as weight tying can reduce in parameter counts without reducing the amount of computation \cite{lan2019albert}. 

        %Number of FLOPs is a common measure used to evaluate the amount of computation required by a model. 
        Optimizing for FLOP counts has motivated the development of model architectures that achieve comparable task performance under a fixed FLOP budget \cite{dai2020funnel} and scaling model width and depth to reduce overall size \cite{sanh2019distilbert}. Low-FLOP operations, such as grouped convolutions \cite{iandola2016squeezenet, zhang2018shufflenet} and inverted residual bottlenecks \cite{sandler2018mobilenetv2, sun2020mobilebert}, have been developed as substitutes for their standard, dense counterparts.  However, the tensor operation primitives and underlying hardware support varying levels of parallelism for different arithmetic operations, leading to low correlation between FLOPs and latency.

        % From the perspective of device utilization, hardware and model FLOPs utilization are reported as the ratio between observed FLOPs per second and a hardware platforms peak theoretical FLOPs. 
    
        % Finally, Critical Datapath Length (CDL), or model depth, corresponds to the number of required tensor operations in a model \cite{langerman2020beyond}. 
        % CDL assumes that parallelizable layers will be run in parallel -- in practice this rarely holds as layers are executed as separate kernel calls.
        % However, for single example inference, CDL has been shown to have a higher correlation with model latency on GPU than number of FLOPs. Previous work where CDL was tested with Vanilla PyTorch limited analysis to examples of batch size one in the inference setting.
    
        Previous works examining the relationship between the mentioned efficiency measures have shown that these metrics often do not correlate well with each other, nor with direct measurements of latency in large scale training \cite{dehghani2021efficiency, wang2020systematic}. We extend this analysis to this inference setting and show that some of these metrics breakdown entirely due to additional performance bottlenecks that emerge at different scales of computation. 

        % There are good reasons for the community to search for simple numerical measures of efficiency.  
        % AutoML and Neural Architecture Search (NAS) allow for automatic efficient model design by optimizing jointly for FLOP count and accuracy. Such scores can be customized depending on the researchers' constraints.  For example, hardware-aware approaches directly incorporate latency or energy usage into the NAS search objective \cite{wu2019fbnet, tan2019mnasnet,wang2020hat}. While manual inspection of the learned models shows that NAS often implicitly learns to take advantage of supported parallelism (i.e. learning wider architectures on GPU devices and deeper models on CPU devices) \cite{cai2018proxylessnas,tan2019mnasnet, sandler2018mobilenetv2}, to our knowledge these measures of inference speed are determined wi


\subsection{Hardware and Platform Performance Analysis}
    Efforts to establish common benchmarks leverage reference models and hardware platforms with target latency or accuracy \cite{reddi2020mlperf,janapa2022mlperf, zhou2020hulk}. Although these efforts have led to improvement in end-to-end latency, they often abstract away the underlying frameworks, compilers, backends, and hardware platforms. While general purpose improvements in hardware and software kernels may lead to improvements across all models, it has been argued that solely focusing on performance optimization of a limited set of model architectures and runtimes may lead to overspecialization \cite{hooker2020hardware}.

    Previous analysis of the computational properties of hardware accelerators has largely focused on the training setting in which larger kernels and batch sizes hide framework overhead that emerges in the inference setting \cite{wang2020systematic, zhu2020daydream, zhu2018tbd}. Analyses of overhead in machine learning systems has primarily focused on domain-specific applications, such as reinforcement learning and recommendation systems settings \cite{gleeson2021rl, lin2022building}, where simulation and memory access dominate execution time. These prior efforts are largely restricted to a small set of reference model architectures and have not directly examined the relationship between model and platform in inference across scale.
    

    
% Early deep learning frameworks, such as Caffe \cite{jia2014caffe}, Theano \cite{al2016theano}, and Tensorflow \cite{tensorflow2015-whitepaper}, were developed under an explicit graph and define-and-run paradigm in which computational graphs were built explicitly and then compiled ahead of runtime. In contrast, modern deep learning frameworks, such as PyTorch \cite{paszke2019pytorch} and TensorFlow Eager, are primarily developed under an eager execution, define-by-run paradigm. Eager, in which the computational graph is built by composing operations in the local environment, is favored for its use and debugging. However, this flexibility comes at the cost of additional overhead by executing the computational graph as defined. 

% High-level frameworks abstract away implementation of the underlying tensor operations to linear algebra and neural network packages which implement basic matrix primitives, such as: CUDA and CuDNN on Nvidia GPUs, OneDNN on Intel CPUs, NNPack, OpenBLAS, or Eigen. Depending on input sizes and formats these libraries will select different  algorithms for implementing the matrix operations, such as deciding between FFT, GEMM, winograd for 2D-convolutions. These libraries provide interfaces for execution of tensor operations using vector instruction sets such as AVX and SSE on Intel CPUs, and NEON instruction on ARM CPUs.

    % For ease of development and debugging, high-level frameworks default to an eager-execution approach to graph construction. Just-in-time compilers such as TorchScript and Torch.fx allow for acceleration of computational graphs by fusing redundant operations into a single computation, such as fusion of convolutions and batch norm layers. By completely exiting the high-level framework, models can be accelerated by exporting into inference-specific runtimes such as ONNX. ONNX is a platform agnostic interface for serializing computation graphs into a common format that can be run using a variety of backend execution providers such as: CUDA and TensorRT on Nvidia GPUs, OpenVINO on Intel CPUs, ARM NN on ARM CPUs.  


    


==> sections/3_preliminaries.tex <==
% \usepackage{multirow}


    \begin{figure}
         \centering
         \includegraphics[width=0.45\textwidth, trim=0cm 5cm 0cm 0cm]{assets/assets-1/execution.pdf}
         \caption{Example profile of a model where runtime is bound by CPU-framework operations (above) and bound by GPU kernel operations (below). Small compute kernels are common at lower batch sizes and in inference. Boxes with dashed lines represent \textit{framework overhead}. }% as defined in \S\ref{sec:framework-overhead-defn}.}
         \label{fig:framework-boundedness}
         \vspace{-20pt}
    \end{figure}
    
\section{Preliminaries}
% maybe combine captions into one caption for the figure -emma
%true
% can't figure out how to make the second one stop being allergic to the first tho
%     \begin{figure}
%          \centering
%          \includegraphics[width=0.49 \textwidth, trim=0cm 5cm 0cm 0cm]{assets/assets-1/execution.pdf}
%          \caption{Example profile of a model where runtime is bound by CPU-framework operations (above) and bound by GPU kernel operations (below). Small compute kernels are common at lower batch sizes and in inference. Boxes with dashed lines represent \textit{framework overhead} as defined in \S\ref{sec:framework-overhead-defn}.}
%          \label{fig:framework-boundedness}
%     \end{figure}
% \vspace{-5pt}


\subsection{Neural Network Frameworks and Runtimes}  
    Specialized frameworks enable execution of deep learning workloads by implementing and providing APIs for tensor operations, gradient calculation, and construction of the network's computational graph.  Frameworks generally fall into the following design paradigms \cite{kahn2022flashlight}:
    % \vspace{-5pt}
    \begin{itemize}[leftmargin=*]
        \item \textbf{Eager Execution}: A computational graph is constructed from a series of operations that are executed as soon as they are called from an interpreter. Examples include: PyTorch \cite{paszke2019pytorch}, TensorFlow 2.0 Eager \cite{tensorflow2015-whitepaper}, Chainer \cite{tokui2015chainer}. 
        \item \textbf{Deferred Execution}: A series of operations are defined and then executed on sample data to generate a full dataflow graph that can then be just-in-time (JiT) compiled. Examples include: PyTorch TorchScript, Jax \cite{jax2018github}, Theano \cite{al2016theano}, Caffe \cite{jia2014caffe}.
        \item \textbf{Static}: A computational graph is pre-defined, compiled, and executed inside a specialized runtime. Fully static computation graphs allow for aggressive, global ahead-of-time compiler (AoT) optimizations. Examples include: ONNX Runtime, TensorFlow 1.0, MXNet \cite{chen2015mxnet}, Nvidia TensorRT, and TVM \cite{chen2018tvm}. 
    \end{itemize}
    % \vspace{-10pt}
    While naively, the deferred and static settings appear to provide obvious benefits in production settings -- the machine learning research community continues to rely heavily on eager mode frameworks for their ease of use.  This further exacerbates the community divide, where models are designed under different assumptions than deployed. 
        
    Deferred and static execution frameworks leverage JiT or AoT compilation of their computational graphs allowing for optimizations such as operator fusion. However, they are limited in model expressivity due to reduced support for structures such as control flow and dynamic input sizes. In contrast, models under the eager execution paradigm allow for more flexibility but incur larger amounts of framework overhead running inside an interpreted environment. 

    % Remove?
    % Graph optimization can still be applied to eagerly defined models by later applying compilation methods. For example, PyTorch models can be JiT-compiled with TorchScript to transform eager-mode models into intermediate representations (IRs) that run independent of Python dependencies. Likewise, PyTorch models can be AoT compiled and executed in the ONNX runtime. These post-hoc compilations provide access to graph optimizations and compatibility with multiple backend execution providers (e.g. CUDA, TensorRT, TVM, etc.). % Execution with these precompiled models and inference runtimes can substantially reduce framework overhead at the cost of less support for operations and a more complex user experience.     
    


   \begin{figure}
     \centering
     \includegraphics[width=0.4\textwidth]{assets/assets-1/framework-overhead.pdf}
     \caption{Framework overhead of ResNet-50 in PyTorch for various batch sizes on an RTX-8000. Framework overhead is substantial at low batch sizes but only a small constant at large batch sizes.}
     \label{fig:framework-overhead}
    \end{figure}
    
\subsection{Framework Overhead}
\label{sec:framework-overhead-defn}
    % Question: Should this be in log log scale?
    % \begin{figure}
    %      \centering
    %      \includegraphics[width=0.35\textwidth]{assets/assets-1/framework-overhead.pdf}
    %      \caption{Framework overhead of ResNet-50 in PyTorch for various batch sizes on an RTX-8000. Framework overhead is substantial at low batch sizes but only a small constant at large batch sizes.}
    %      \label{fig:framework-overhead}
    % \end{figure}
    \begin{figure*}[ht!]
        \includegraphics[width=1\textwidth]{assets/assets-1/baselines-new.png}
        \vspace{-5pt}
        \caption{Latency vs. batch size for baseline models in FP16 and FP32 on RTX-8000. Framework boundedness exists for all models at small batch sizes where framework overhead dominates runtime regardless of Framework overhead is most prominent in smaller models executed in half precision (FP16) on slower frameworks.}
        \label{fig:baselines}
        \vspace{-5pt}
    \end{figure*}    
    
    % TODO: Complete this table
    \begin{table}[ht!]
    % \vspace{-10pt}
        \small
        \centering
        \begin{tabular}{@{}ccccccc@{}}
         \textbf{Batch}  & \multicolumn{2}{c}{\textbf{PyTorch}} & \multicolumn{2}{c}{\textbf{TorchScript}} & \multicolumn{2}{c}{\textbf{\textbf{ONNX RT}}}  \\
         \textbf{Size}  & \textbf{FP32}    & \textbf{FP16} & \textbf{FP32}  & \textbf{FP16} & \textbf{FP32}  & \textbf{FP16}    \\  \toprule
          1              &  48.52 & 16.09        &  79.66             & 18.11    &  92.20 & 41.34   \\ %\hline
          % 2              &  77.58 & 20.57        &  79.86             & 22.56    &  93.82 & 51.99    \\ %\hline
          % 4              &  83.20 & 29.21        &  84.55             & 33.81    &  93.60 & 75.73     \\ %\hline
          8              &  88.22 & 75.87        &  87.86             & 43.51    &  96.28 & 90.91    \\ % \bottomrule
          16             &  90.34 & 84.43        &  90.79             & 77.31    &  97.72 & 94.51     \\
          32             &  93.35 & 90.71        &  92.18             & 93.28    &  98.90 & 97.34               \\ 
          64             & 94.97  & 93.21        &  93.02             & 94.06    & 99.40 & 98.81 \\
          % 128            & 95.49  & 95.14        &  94.206            & 94.42    & 99.62 & 99.53 \\ \bottomrule
        \end{tabular}
    	\caption{Percentage of total inference latency spent on GPU execution time, reported for ResNet-50 on an RTX-8000. At low batch sizes, the proportion of time spent on GPU execution is lower; this is especially apparent for FP16 computation, where even TorchScript and ONNX exhibit substantial framework overhead.}
        \label{tab:gpu-util}
    \end{table}
    
  %  \begin{table}
  % \small
  % \centering
  % \begin{tabular}{@{}c@{\hspace{1em}}c@{\hspace{1em}}c@{\hspace{1em}}c@{}}
  % %\hline
  % \textbf{Batch}	& \textbf{PyTorch} & \textbf{TorchScript} &  \textbf{ONNX (CUDA)} \\ \toprule
  % \phantom{0}1  & \phantom{0}5.816   &   \phantom{0}4.445  &  \phantom{0}3.058  \\ %\hline
  % \phantom{0}2  & \phantom{0}6.084   &   \phantom{0}4.645  &  \phantom{0}3.334  \\ %\hline
  % \phantom{0}4  & \phantom{0}6.103   &   \phantom{0}4.688  &  \phantom{0}5.268  \\ %\hline
  % \phantom{0}8  & \phantom{0}9.376   &   \phantom{0}7.641  &  \phantom{0}7.332  \\ %\hline
  % 16            & 16.790             &  13.027             &  12.217  \\ %\hline
  % 32            & 31.936             &  24.052             &  23.931  \\ %\hline
  % 64            & 62.523             &  46.688             &  45.979  \\ %\hline
  % \bottomrule
  % \end{tabular}
  % 	\caption{Latency (ms) of ResNet-50 across frameworks. For low batch sizes, latency is constant in PyTorch and TorchScript, but is optimized for all batch sizes in ONNX.}
  %   \label{tab:gpu-latency}
% \end{table}
    In practice, deep learning frameworks leverage highly parallelized hardware accelerators, most commonly GPUs, to increase the speed of computation. To execute computation on an accelerator, frameworks dispatch kernel calls from a host-device CPU to execute asynchronously on the GPU accelerator as shown in Figure \ref{fig:framework-overhead}. In Table \ref{tab:gpu-util}, we observe that small inference workloads demonstrate low GPU \textit{compute utilization} \cite{zhu2018tbd}, the difference between total execution time and active GPU time. Profiling shows that this suboptimal utilization is due to the rapid execution of small computer kernels is not enough to saturate the fixed cost framework overhead from time spent on CPU operations to launch appropriate kernels, construct computational graphs, handle control flow, and device synchronization. 

    % In large scale training settings, computation of gradient and large batch sizes result in compute kernels that dominate the total execution time of the model. In contrast, small batch sizes in inference settings produce relatively small compute kernels that execute very quickly.
    
    % We formalize this concept with as \textbf{framework overhead} the difference between the total execution time for a forward pass through the network and the time spent executing accelerator kernels. Similar to model FLOPs utilization \cite{chowdhery2022palm}, which measures how well a model utilizes its available hardware, framework overhead reflects how efficiently a model can enqueue computation to available hardware. 

    As some CPU and GPU operations must be synchronized and executed in order (such as in the setup of the computational graph and the first kernel launch), all models have sub-optimal GPU compute utilization and positive-value framework overhead. 
    However, framework overhead becomes much more prominent when the GPU compute kernels execute quickly but overall execution is blocked by CPU framework operations for setting up and dispatching kernel calls (see Figure~\ref{fig:framework-boundedness}).  
    When the execution of almost all GPU kernel computation is being blocked on framework operations, the model's execution becomes \textit{framework-bound}. That is, latency is entirely dependent on the runtime of setup operations and CPU kernel dispatch calls. As a result, latency is constant regardless of batch size or number of MACs computed. For settings in which latency is dependent on the execution of computational kernels and data movement, we refer to models as being \textit{compute-bound}.

   \begin{figure}
        \centering
        \includegraphics[width=0.3\textwidth]{assets/assets-1/baseline_avgmacs-new.png}
        \label{fig:baselines-avgmacs}
        \caption{Average MACs per layer vs. latency. Model that rely on standard convolution and linear operations transition to compute-boundedness at similar number of \textit{average} MACs per layer} 
        \vspace{-15pt}
    \end{figure}
    


    
    %Neural scaling laws provide guidance for setting parameter counts for a given training compute budget as measured in petaflop days (PF-Days) \cite{kaplan2020scaling}. 
     %However, the tensor operation primitives and the underlying hardware support varying level of parallelism support for different types of arithmetic operations, leading to poor correlation between FLOPs and latency. %% This  is redundant to earlier

% \section{Experimental Setting}
% We select a range of commodity hardware platforms including GPUs, such as the V100 and A100s, which are commonly found on consumer cloud computing platforms as of the time of submission. 
% \subsection{Hardware Platforms}

%     \subsubsection{Server Platforms}
% %     We perform CPU-only evaluations on Intel Xeon-W2295 with support for AVX-2 and AVX-512 vector extensions with 36 cores and 256 GB of RAM. Runtime optimizations are provided via oneDNN AVX-2 and AVX-512 extensions enable parallel execution of 8 and 64 single-precision FLOPs per clock cycle.
%      GPUs with support for CUDA and the cuDNN matrix library are among the most common hardware accelerators used for execution of neural network computational. We survey the performance of GPUs across a variety of recent Nvidia microarchitectures, evaluating on Titan X and 1080 Tis from the Pascal architecture; RTX-8000, V100s, and 2080 Tis of the Volta-Turing Architecture; 3090 and A6000s from the Ampere architecture. Full GPU details are provided in \ref{Tab:Hardware Platforms}.  Tensor core accelerations are enabled for half precision (fp16) operations on Volta architectures, and for both half and single precision (fp32) operations on Ampere architectures. 

%     Experiments were conducted on compute nodes allocated 32 GB of RAM within a distributed slurm cluster. Compute node CPUs included: 32-core AMD EPYC 7502 for A100 nodes, 16-Core AMD EPYC7282 for 3090 nodes; 8-core Intel Xeon Silver 4110s for the 1080 Ti and A6000 nodes; and 8-core Intel Xeon E5-2630 for the Titan X, 2080Ti and RTX-8000 nodes. 
    
% \subsection{Models}
    
%     \textbf{Language Models}: 
%     State-of-the-art natural language processing (NLP) models are largely based around the self-attention encoder architectures such as BERT \cite{devlin2018bert} inspired by the Transformer nerual network paradigm \cite{vaswani2017attention}. 

%     % Why these models?
%     In addition to the vanilla BERT model, we evaluate across models inspired by the BERT architecture that modify its architecture to target efficiency. In particular, we examine DistilBERT \cite{sanh2019distilbert}, SqueezeBERT \cite{iandola2020squeezebert}, MobileBERT \cite{sun2020mobilebert}, AlBERT \cite{lan2019albert}, and Funnel Transformer \cite{dai2020funnel}. Pretrained models were sourced from HuggingFace.
    
%     \textbf{Vision Models}
%     Computer vision applications commonly leverage both convolutional neural network and transformer based architectures. Specifically, we perform evaluations on common baseline models: ResNet-[18, 50, 101, 152] \cite{he2016deep}, Inception Net \cite{szegedy2016rethinking}, DenseNet \cite{iandola2014densenet}, and ViT-32 \cite{dosovitskiy2020image}. Additionally, we examine efficient architectures discovered via neural architecture search: 
%     EfficientNet V2 \& EfficientNet Lite \cite{tan2019efficientnet}, MobileNet v2 \cite{sandler2018mobilenetv2}, and MnasNet \cite{tan2019mnasnet}. We also examine ShuffleNet \cite{zhang2018shufflenet} and SqueezeNet \cite{iandola2016squeezenet} which replace standard convolutions with lighterweight grouped and squeeze variants.
    
%     Pretrained models were sourced from Timm and torchvision, as available.
    
% \subsection{Frameworks and Runtimes}
%     We evaluate models executed in PyTorch, TorchScript, and ONNX Runtime with the CUDA backend. We select PyTorch as representative of eager-execution based frameworks that incur framework overhead from both its Python language dependency and from unoptimized kernel launches.    
    
%     We select TorchScript as a representative case of just-in-time compilation optimizations over standard PyTorch and removal of the Python language overhead. TorchScript provides basic performance optimizations including: loop unrolling, fusion of element wise operations, and dead-code elimination; but minimal graph optimizations \cite{devito2022torchscript}.
    
%     We also evaluate models in the ONNX runtime with a CUDA execution provider as a backend. The ONNX inference runtime is a representative case of ahead-of-time-compilation with a static computational graph, and provides several level of graph optimizations.
    
%     % Due to device limitations, models are implemented with PyTorch 1.9.0 with CUDA 10.2 on Python 3.6.9 on the Jetson Nano.
        

% \section{Methodology}
%     For each model, framework and hardware platform we measure the latency, memory utilization, GPU utilization, and number of multiply-accumulate operations (MACs).  Latency measurements are recorded as the average time for execution of 100 forward pass iterations following an initial warmup used to initialize the model weights and data. GPU utilization was measured using PyTorch's built-in profiler. GPU memory utilization was measured with NVML. 

%     We evaluate on batch sizes from 1 to 128 to cover a range of real-world use cases. Increasing batch size is a common method for improving GPU utilization. Single example inference, with batch size of 1, is common for many on-device applications in which inference is being performed real time such as in autocomplete and real-time automatic speech recognition. Inference on larger batches is also deployed in real-time settings such as in the processing of multiple concurrent frames in a vision system in remote sensing or on an autonomous vehicle.  Batched inference for extremely large sample counts is also common in offline server settings.

%     For vision models, input data was fixed at 224 x 224 rgb images the NCHW format. For language models, input data were sequences of length 128 of the shape Nx128. All data was randomly generated.

    % \subsection{Analysis Methods}
    % % Analysis: latency as a function of GPU util, batch size, Total MACs, and MACs per layer, NN Calls, Roofline
    % % Situations:
    % %   - Frameworks
    % %   - Optimizations: Precisions
    % %   - Model Architectures: 
    % %       - Groups: Standard CNNs/TFs, Mobile Networks, Heterogeneous layers

    
    % First, we analyze how different frameworks impact latency and throughput as a function of 
    % \textbf{Latency vs. Batch Size.} We examine latency as a function of batch size to reflect the relationship between the \textit{number of samples processed} and model execution time.

    % % \textbf{Latency vs. Memory.} We examine latency as a function of the size of memory allocated for the model and weights by the GPU. 

    % \textbf{Latency vs. Total MACs.} We examine latency as a function of the Total MACs to reflect the relationship between the \textit{total amount of computation performed} and model execution time. 

    % \textbf{Latency vs. Average MACs per Layer.} We examine latency as a function of the average number of MACs per layer. 

    
    % We then extend these analyses across various model architectures.

    % W

% \label{Appx:Platforms}
% Table 1: Hardware Platforms
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
 

==> sections/4_analysis.tex <==
\section{Experimental Setting}    
    % The two most prevalent architectures in state-of-the-art models for computer vision and natural language processing are build on variants of the convolutional neural network and Transformer \cite{lecun1989handwritten, vaswani2017attention}. 
%  Due to their widespread usage, the underlying convolution, self-attention, and linear operations that constitute these models are fairly standardized with strong support across frameworks and hardware platforms. 

    % \todo{Clarify that in overhead figures like Figure 1, the CUDA kernel execution time is an upper bound if the profiler introduced any overhead --- therefore, it's a lower bound on the gap between wall clock and GPU time}

    
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{assets/assets-1/model-scaling.png}
    \label{fig:model-scaling}
    \vspace{-5pt}
    \caption{Comparison of latency for BERT and ResNet variants that scale model \textit{width} and \textit{depth}. Increases in model depth add more framework overhead, whereas increases in model width lead to faster transitions to compute boundedness. ResNet-50 and its Wide ResNet-50 variant are equivalent in latency up to batch size 8 despite having over 3x fewer parameters. }%Intuitively, as a result, increases in floating point operations resulting from wider network widths cause smaller increases in latency than those resulting from larger batch sizes. \textcolor{red}{review pls bc this was clara lol}}
\end{figure*}    

    Models are executed with frameworks from each of the major paradigms: PyTorch (eager execution), just-in-time compiled TorchScript (deferred), and ahead-of-time compiled ONNX Runtime with a CUDA backend (static).  PyTorch models are executed with eager execution, which incurs substantial added overhead from Python language dependencies. In contrast, TorchScript allows for execution in a Python-free environment and provides basic compiler optimization. % in the form of dead code elimination and fusion of element-wise operations. 
    The ONNX runtime provides full ahead-of-time compilation with support for computational graph optimizations. % and removal of redundant operations such as kernel fusion of GEMM and Conv layers with subsequent normalization and activation layers.
    
        We evaluate over a range of batch sizes to capture common inference use cases as stated in \cite{reddi2020mlperf}: single example inferences is common in streaming on-device applications, such as autocomplete and automatic speech recognition; larger batch-size inference is deployed in real-time settings such as in the processing of multiple concurrent frames on an autonomous vehicle; extremely large batch inference is typical in offline server settings.

    We measure latency as the average time for execution of 100 forward passes (following 10 warm-up passes to initialize model weights and data). GPU core and memory utilization are measured with PyTorch's built-in profiler and NVIDIA Management Library (NVML), respectively. We randomly generate image input data as 224 x 224 RGB images in NCHW format, and language data as random embedding sequences of length 128.   


\label{sec:baselines}



\section{Model Design Decisions}
We examine a variety of efficient model architecture design decisions and investigate their alignment with commonly reported efficiency proxies and empirically observed latency. 

\subsection{Baseline Models}
    We select ResNet-50 \cite{he2016deep} and BERT-Base \cite{devlin2018bert} as representative architectures of the convolutional neural network and transformer neural network architecture paradigms commonly used in natural language processing and computer vision. Both models are commonly used in deployment settings and are found in major machine learning benchmarks \cite{reddi2020mlperf}.
    
    % \subsubsection{Analysis} 
    % General Explanation 
    The number of FLOPs required for model inference scales linearly with the input batch size. As such, one would expect that latency scales accordingly as well. However, as seen in Figure~\ref{fig:baselines}, both ResNet-50 and BERT-Base exhibit framework boundedness at small batch sizes, where latency is constant regardless of batch size. 
    
    Framework boundedness exists for inference with both single (FP32) and half precision(FP16). As the half precision computation is slower due to reduced data movement, GPU kernel execution time takes longer to overtake fixed framework overhead leading FP16 inference to be framework bound until larger batch sizes. 
     We can see that with single precision, BERT and ResNet-50 are framework-bound by PyTorch up to batch sizes 4 and 8, respectively. However reducing to half precision leads both of these models to remain framework-bound by PyTorch up to batch size 16. For inference with larger compute-bound batch sizes, we observe the expected speedups from using half precision, with the PyTorch FP16 latency of ResNet-50 and BERT being faster at batch size 128. %These effects are more pronounced on older pre-Ampere Nvidia GPUs, such as the 1080Ti, which do not implement efficient FP16 Tensor Core operations. % Reference table in the back

    % Models with more concurrent operations tend to be less framework-bound
    While both BERT and ResNet-50 exhibit framework-bound behavior, they transition to compute boundedness at different batch sizes. The difference in model behavior can be attributed to the fact that they saturate their compute kernels at different rates. Framework-boundedness is mainly determined by whether the number of operations being executed takes longer than the dispatching CPU operations. For the well-optimized operations (Conv2Ds and GEMMs) that make up ResNet-50 and BERT, the time per FLOP is reasonably consistent.   


\subsection{Scaling Model Depth \& Width}
    \begin{figure*}[!ht]
        \centering
        \includegraphics[width=\textwidth]{assets/assets-1/model-mobileops.png}
        \vspace{-10pt}
        \caption{Latency of CNN and Transformer models using \textit{efficient variations} of convolution and self-attention operations. All of the variants observe lower latency at large batch sizes, but have worse FLOP utilization. Efficient Transformer variants are slower than BERT at small batch sizes due to the introduction of more layers. See Fig~\ref{fig:bs-efficient-bert} in Appendix~\ref{appx:figs} for batch size comparison in BERT models}. % TODO: Clean up this sentence
        \label{fig:model-mobileops}
    \end{figure*}    
    
    \begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{assets/assets-1/model-pooling.png}
    \vspace{-10pt}
    \caption{Comparison of latency for BERT and Funnel Transformer. Despite using fewer total MAC operations, Funnel Transformer is slower than BERT for inference due to the introduction of additional intermediate pooling layers. }
    \label{fig:model-pooling}
    \end{figure}
    
    \begin{figure*}[!ht]
        \centering
        \includegraphics[width=\textwidth]{assets/assets-1/hardware-new.pdf}
        \vspace{-25pt}
        \caption{Framework overhead occurs across multiple generations of GPU hardware –- increasingly prominently with newer generations. See Fig~\ref{fig:throughput-gpu} in Appendix~\ref{appx:figs} for an alternative view featuring throughput across generations of GPUs} % TODO: Clean up this sentence
        \label{fig:hardware}
    \end{figure*}
    

    
    % Figure: Latency vs Batch Size and MACs for ResNets and BERt
    \subsubsection{Assumption}
     Depth and width scaling have been applied to CNN and Transformer architectures 
    in NLP and vision as a means of increasing end-task accuracy \cite{he2016deep, touvron2021going, zhou2021deepvit}. Recent work has shown that model end-task performance scales differently along each axis \citep{tay2021scale, tay2022scaling} and end-task performance at the example level can differ depending on the axis
    %different performance qualities can be observed at different scales 
    \cite{nguyen2021do}. 
    
     We compare our baseline models to variants that scale both model width and depth. For ResNet-50, we examine against ResNet-18, 101, and 152 \cite{he2016deep} which each scale the number of residual blocks, and Wide ResNet-50 \cite{zagoruyko2016wide} which increases the model's channel widths. Similarly, we examine 12-layer BERT-Base against its 6-layer DistilBERT \cite{sanh2019distilbert} variant and experiment across parameterized BERT models, varying the number of encoder layers as well as width of their fully connected and self-attention layers. 


    \subsubsection{Analysis}
    % From the perspective of throughput
    When scaling model depth and increasing number of layers, latency increases in both the framework- and compute-bound regimes as each added layer operation requires an additional CPU-GPU dispatch. ResNet and BERT variants have a larger fixed latency in the framework-bound regime for larger numbers of layers and scale similarly with batch size in the compute-bound regime, as seen in Figure~\ref{fig:model-scaling}.
    

    Counter-intuitively, the wider variations of ResNet-50 and BERT see \textit{no increase in latency} at low batch sizes. As this computation is framework bound, total runtime is constant despite the wider operations requiring more floating point operations. Instead, however, increased kernel execution time causes these wider models to become compute-bound at lower batch sizes. Once in the compute-bound regime, latency scales more rapidly with batch size for wide models.
    
    To best utilize hardware for inference with low batch sizes, model width can be freely scaled until the compute kernels saturate enough to exceed the kernel launch costs. In practice, the hidden dimensions of both BERT and ResNet-50's largest and most computationally intensive linear and convolution layers can be doubled without affecting the single-example latency speed. 

    % While model depth and width provide insight into the framework overhead for a given model, the actual wall clock latency 
    % TODO: Discuss how scaling affects latency for compute bounded models
    % Exactly determining framework overhead is difficult as it is the product of Model X Framework X Hardware 



\subsection{Downsampling and Hierarchical Pooling}
    \subsubsection{Assumption}
    Self-attention layers in Transformer architectures are notoriously computationally expensive as their computational complexity scales quadratically as a function of input sequence length. To reduce this computational bottleneck, researchers have developed a efficient transformer architectures that downsample the sequence to reduce length and total MACS, such as Swin and Funnel Transformers~\cite{dai2020funnel, kitaev2020reformer, wang2020linformer}.  

    We examine the performance of a Funnel Transformer variation that applies average pooling every 4 layers. The model achieves comparable accuracy to BERT on downstream tasks while requiring $42\%$ fewer total MAC operations through sequence length reduction. This model achieves similar downstream task performance to BERT-Base and trains $33\%$ faster based on wall-clock time.
    
    \subsubsection{Analysis}
    While Funnel Transformer reduces total FLOPs to obtain substantial speedups in large-scale training, this speedup does not translate to increased speed of inference as seen in Figure~\ref{fig:model-pooling}. In practice, the average pooling layers used to perform sequence length reductions add additional operations to the computation graph and increase the model's framework overhead. At low batch sizes, Funnel Transformer is framework bound at a much higher latency than BERT and remains slower even at larger batch sizes. For framework bound models, inclusion of additional layers increases overall latency even if reducing total number of FLOPs.  

    % \begin{figure*}[!ht]
    %     \centering
    %     \includegraphics[width=\textwidth]{assets/assets-1/hardware-new.pdf}
    %     \vspace{-15pt}
    %     \caption{Framework overhead occurs across multiple generations of GPU hardware –- increasingly prominently with newer generations.} % TODO: Clean up this sentence
    %     \label{fig:hardware}
    % \end{figure*}
    

\subsection{Efficient Mobile Operations}
    \subsubsection{Assumption}
    Model architectures that target deployment on edge devices, such as mobile phones, are often designed to decrease the total number of FLOPs or MACs under the assumption that such reductions translate to decreased latency in deployment. Towards this end, operations such as grouped convolutions \cite{zhang2018shufflenet}, inverted residual bottlenecks (MBConvs) \cite{sandler2018mobilenetv2}, and squeeze and excitation layers \cite{iandola2016squeezenet} have all been proposed as substitutes for larger dense convolution and linear operations. However, in practice these operations often lack the highly optimized framework and hardware support developed for more standard operations and as a result exhibit higher per-flop latency and poor memory utilization.

    We examine this assumption with models that use grouped convolutions in SqueezeNet \cite{iandola2016squeezenet} and SqueezeBERT \cite{iandola2020squeezebert}, and models that use inverted bottleneck layers in EfficientNet-Lite \cite{tan2019efficientnet}, MobileNet \cite{sandler2018mobilenetv2}, MNAS Net \cite{tan2019mnasnet}, and Mobile BERT \cite{sun2020mobilebert}.
    
    % These operations largely tradeoff dense computation that executes over the entire input by operating on only some of the input features (e.g. grouped convolutions), factorizing convolution into separate depthwise and pointwise convolutions (e.g. MBConvs), or by bottlenecking the model and reducing the size of the feature maps (e.g. Squeeze and Excite Layers). 

    % Explain these operations ?
    % SE: Reduces computation by bottlenecking and compressing layers with large number of activations
    % MBConv: Factorizes computation of multichannel convolutions
    % Grouped Convolutions: Convolution over a subset of these 
    
    \subsubsection{Analysis}
    CNNs using grouped convolutions and MBConv operations yield the desired decreased latency compared to ResNet-50 while achieving similar or better downstream accuracy. However, the models that use these operations exhibit worse FLOPS throughput due to poor memory utilization as seen in Figure~\ref{fig:model-mobileops}. % Cite? 
    Additionally, these operations can suffer in deployment settings where component depthwise and pointwise convolutions may have limited hardware and framework backend support.  

    Likewise, Transformer models also use several inverted bottlenecks and grouped convolutions as substitutes for self-attention layers. Similar to pooling operations, this introduces substantial framework overhead that slows down execution for low batch sizes. However, at large batch sizes, reduction in FLOPs yields empirical wall-clock gains over a BERT baseline.

\section{Framework Considerations}
    % Deep learning frameworks provide usable APIs to construct neural networks and abstractions over underlying primitives. Modern frameworks task themselves with managing the execution, construction, and optionally compilation of the computation graph.
    Frameworks adhering to an eager mode of graph construction, such as PyTorch or TensorFlow 2.0, incur overhead from execution inside an interpreted environment given that the time between kernel launches is related to the speed at which kernels are enqueued, which is in turn affected by host-side latency. To mitigate this, inference frameworks such as TorchScript attempt to reduce interpreter overhead and introduce computation graph-level optimizations. 
    %In particular, TorchScript provides serialization of PyTorch models and basic compiler optimizations such as dead code elimination and constant folding.
    Static runtimes can remove interpreter overhead entirely by compiling graphs ahead of time; the ONNX runtime provides further optimizations through graph rewrites that can fuse operators such as GEMMs and convolution layers with subsequent activations or norms. Such fusion operations can reduce memory footprint and result in more efficient kernels, decreasing overall framework overhead.
    
    % Faster frameworks yield less framework overhead
    Unsurprisingly, model latency decreases when performing inference with frameworks and runtimes that support more aggressive optimizations as seen in Figure \ref{fig:baselines}. These increases are especially pronounced at low batch sizes where inference is framework-bound. For batch size 1, TorchScript and ONNX provide an average FP16 speed up of 34.16\% and 71.38\% over PyTorch, respectively. As batch sizes increase and models become compute bound, there is substantially less difference in latency across frameworks as the majority of execution time is spent awaiting the completion of kernel execution.
    
    % fp16 ONNX -- 128 -- 9.45 sec latency with all , torchscript 4.0299 seconds 
    % Kernel quality across computation models and frameworks also has a significant impact on performance. In particular, high-quality code generation of operator implementations on accelerators can improve performance, even for the same GPU utilization. Given this, utilization is a relatively poor proxy for assessing high-level performance. % For a saturating batch size of XX on [hardware YY], ONNX, which has negligible framework overhead due to its precompiled graph, 

    Although these speedups suggest that inference should always be executed in specialized inference frameworks, in practice, frameworks with lower overhead can still be slower than more costly frameworks due to variations in kernel selection, code generation, and operator support.
    % or limited support for component operations. Inference runtimes often support only a subset of the available operations in more flexible eager frameworks designed for research and prototyping, and thus require CPU fallback operations. 
    % For example, FNet is a BERT variant which replaces self attention layers with Fast Fourier Transform (FFT) operations. Although FFTs are deterministic operations with good hardware support, they are not in the ONNX opset. In this case, FNet executed with eager PyTorch is still XX ms faster than BERT despite using a less optimized framework. 
    Additionally, custom frameworks can often lag the research community and lack support from the most recent libraries implementing matrix primitives. For example, PyTorch is released with CUDA 11.6 at the time of writing. By comparison, ONNX Runtime only supports CUDA 11.4. Each framework can differ in terms of the quality and choice of the kernels in the backend libraries they utilize for matrix operations, and this can also impact the translation from FLOPs to latency. %  We observe that while the low-batch latency with ONNX is substantially faster than PyTorch and TorchScript, the ONNX Runtime is slower at large compute bound batch sizes which we attribute to it's older version of CUDA which may be leveraging slower compute kernels.  % Cite 

\section{Hardware Considerations}
    In Figure~\ref{fig:hardware}, we observe that framework-bound inference emerges across multiple generations of consumer, workstation, and datacenter Nvidia GPUs. As the speed of the accelerator increases, the relative execution speed of the compute kernels decreases while the total framework overhead due to CPU kernel dispatch operations remains constant. We observe that GPUs that lack Tensor Core support for half precision operations, such as the 1080Ti, are notably slower and less framework-bound than newer GPUs. Conversely, this leads faster GPUs, such as the RTX 3090 and the A100, to remain framework bound at larger batch sizes for both ResNet-50 and BERT. These observations indicate that framework bounds on model execution will continue to worsen as hardware improves unless commensurate improvements are made to deep learning frameworks. For example, BERT-Base is not framework bound for older 1080Ti GPUs but is 
    
    Framework boundedness is mainly caused by bottlenecks due to CPU dispatch operations. As a result, the fixed latency for framework-bound models is a product of the entire system's configuration, dependent on hardware specifications such as the CPU and memory speeds. In contrast, the latency of compute-bound models is mainly determined by the selected kernels and their supported FLOPs per second by the GPU, with faster GPUs yielding faster execution.


% Examination of the runtime profiles shows low GPU utilization of these models for inputs with small batch size; reported in Table \ref{tab:gpu-util}. Until the runtime of the GPU compute kernels is sufficiently large, the overall model's latency is constant blocked by CPU operations managing the computational graph and dispatching kernel launches. Qualitatively, this is observed in runtime profiles in figures \ref{fig:pytorch-profile}, \ref{fig:jit-profile}, \ref{fig:ONNX-profile}. 

% Analysis
% GPU Performance Analysis
% 1. Framework and memory overhead leads to low GPU utilization at small input sizes
% 	- Results in constant time execution
% 	- Layers are a reasonable proxy in the bounded region
% 	- FLOPs are a reasonable proxy in the compute bound region
% 	- Caveats: 
% 		- Graph overhead is dependent on framework, CPU, architecture
%		- FLOP are not entirely predictive of latency; depends on memory locality of operations, type of operation, algorithm, hardware

 
  % 1. Latency vs MACs
  %		0. Latency vs MACs: Doesn't work
  %		a. Find memory bound region: Latency vs Average MACs per layer
  %			- Separate based on highest FLOP layer type
  %			- Exceptions and Other Cases: 
  % 			- Branched Models, 
  % 			- Models with mixed operation types: Efficient Net V2, SqueezeNet, ShuffleNet
  %		b. Plot latency vs total MACs the compute bound region
  % 2. Find latency in the memory bound region
  % 	a. Model Depth
% Comparison Across GPU Architectures
% 	1. NVidia Architecture Generations
%	2. Edge vs Server: CPU and GPU
% Effects of Hardware and Platform Optimization
% 	0. Vector Extensions on CPU:
% 	1. Mixed Precision: Super linear increase in compute
%	2. Tensor Core Utilization: Increases in speeds but model performance is still generally bounded by CUDA core speed
%	3. Model Serialization and JiT: ONNX and Torchscript
    

% In training and at large input sizes, framework overhead is negligible. Hardware utilization is low at small input sizes, which increases the impact of framework overhead on total runtime. For small batch inference settings, eager execution frameworks limit computational efficiency. Actual framework overhead is variable across a number of factors including framework implementation and CPU. 


% \begin{figure*}[!ht] 
%      \centering
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/resnet-bs1.png}
% 		 \caption{ResNet-50 Profile at Batch Size 1 with standard PyTorch.}
%          \label{fig:pytorch-profile}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/jit-resnet-bs1.png}
%         i \caption{ResNet-50 Profile at Batch Size 1 with PyTorch TorchScript.}
%          \label{fig:jit-profile}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{assets/ONNX-resnet-bs1.png}
%          \caption{ResNet-50 Profile at Batch Size 1 in the ONNX Runtime. }
%          \label{fig:ONNX-profile}
%      \end{subfigure}
%     \caption{PyTorch and TorchScript exhibit low GPU utilization for batch size 1 due to blocking on CPU kernel dispatches. ONNX Runtime with the CUDA backend observes high GPU utilization with minimal gaps between kernel execution.}
%     \label{fig:profiles}
% \end{figure*}






% \subsection{Comparison of Hardware Platforms}
% We observe similar patterns of framework bound behavior across multiple generations of Nvidia GPU architectures. Noteworthy, model latency on the Jetson Nano is not obviously framework bound when utilizing an ONNX runtime. This suggests that edge devices achieve reasonably high hardware utilization and low framework overhead due to the limitations of their speed of computation.



% \textbf{Latency in Compute Bounded Regimes}
% After the individual layers have saturated, latency begins to increase linearly according to FLOPs. In this regime, FLOPs are a strong predictor of latency with a Pearson rank correlation of 0.95.

% In figure \ref{fig:GPU_Utilization}, we examine the inference profile of ResNet-50 on an RTX-8000. We observe that for single-example inference there is low GPU utilization as computation is blocked by CPU-operations. Even on efficient models designed for edge devices, such as MobileBert on the Jetson Nano, GPUs fail to achieve high utilization and are blocked by kernel launches.




% TODO: Add figures for BERT (Batch Size and Sequence Length), Res-Net, Inception

% Performance Analysis
% 1. Each operation has a different amount of peak FLOP utilization per platform -- See FLOP utilization heat maps
% 2. Each operation saturates (memory to compute bounds) at a different point -- See roofline
% 3. Operation X Hardware Saturation Point is determined by number of MACs that corresponds to ???
% 4. Memory vs Compute Bound Regime can be determined by:
	% a. Identifying type of operation with the highest number of FLOPs
    % b. 
    % Exceptions: 
% 5. Latency can be determined by:
	% a. Memory Bound Region: Latency is constant regardless of input size 
    
% Model Design Recommendations
% 4. 

% All Parallel Core Architectures Follow Roofline Behaviors
	% Previous work has shown this for single example inference and individual operations
    % Unlike previous work which finds individual operations are memory bound, in the inference setting the model overall is compute bound for most standard input sizes
    % 

% Not all Operations are the same
% While the computational graph creates a more complex transition between memory and compute-boundedness we can approximate it via average MACs in the operationally densest layers (i.e. Conv2D and linear). 
	% Each model observes a different trajectory in both regimes due to differing proportions of operations and layer, framework overhead
    
% Max utilization can be achieved by ensuring input size >= compute boundedness
% Latency is determined by 
% with an \textit{r}-squared value of 0.87 and RMSE of TODO. Similarly, on the Raspberry Pi-4B . 

    
    
% \subsubsection{FLOPS Utilization}
% \label{section:flops-util}
% % TODO : GPU Operations Heatmap
% \begin{figure}
% 	% \includesvg{assets/rtx-floputil.svg}
%     \caption{TODO: FLOPS Utilization RTX-8000}
%     \label{fig:rtx-roofline}
% \end{figure}

% In this section, we investigate the FLOPs utilization at the layer level for fully-connected linear layers, standard 2D convolutions, and factorized inverted bottleneck convolutions. 

% In figure HEAT-MAP, we observe that both 2D-convolution layers and linear layers approach a similar bound on FLOPS utilization. By comparison, the MB-Convolution observes a much lower peak FLOPS utilization due to low arithmetic intensity of its component depthwise-convolution \cite{gholami2018squeezenext}.

% \subsubsection{Memory Bandwidth and Roofline Analysis}
% \label{section:roofline}
% % FIGURE: GPU Roofline Plots
% \begin{figure}
% 	\includesvg[width = 240pt]{assets/rtx-roofline.svg}
%     \caption{Roofline Plot for RTX-8000}
%     \label{fig:rtx-roofline}
% \end{figure}

% In Figure \ref{fig:rtx-roofline}, we show hierarchical roofline plots computed for the RTX-8000. There is a sizable gap between the peak floating point operations per second (FLOPS) and the observed computational intensity of the reported models. 

% We observe that models approach differing peak FLOPS per second. However they approach similar compute bounds on maximum arithmetic intensity as measured in FLOPS.   

       


%  \subsection{CPU Performance Analysis}
% 	Without parallel-core support, model inference is compute bound at all input sizes on CPU-based platforms. In this setting, total latency L and throughput can easily be approximated with a theoretical FLOPs proxy:
%     % $$ \text{Latency} = \frac{\text{Threads} \times \text{Clock Speed}}{\text{SIMD Parallelism}}$$
%     For instance, on Intel Xeon with AVX-2 extensions, supporting 8 concurrent SIMD operations. This baseline model matches ground truth latency recision reduces the memory traffic of operations.
    
    
%     \subsubsection{Just-in-Time Compilation}
%     ONNX and Torchscript

%     % \subsection{Framework Choice}


==> sections/5_discussion.tex <==
\section{Discussion}

\textbf{Using higher-performing hardware does not necessarily improve end-to-end performance.}
Framework overhead limits the impact of improved hardware as it limits utilization. This trend will continue as ML-specific hardware advances without efforts to address software bottlenecks. For example, single-example inference with both BERT and ResNet-50 is slower using an A100 than using a V100 GPU despite a 2.75x increase in peak computational throughput.

\textbf{Tensor computation graph optimizations and compilation improve latency.}
Removal of host Python language dependencies and graph optimizations provides substantial speedups over standard eager frameworks, especially for inference at low batch sizes. However, feature completeness for operators and control flow varies across graph optimizers and JIT compilers. 

For example, the FNet architecture \cite{lee2021fnet} relies on FFTs as a deterministic swap-in for self-attention. FFT operations are not currently supported by ONNX or TorchScript and to our knowledge, no JIT compilers support graph rewrites that add FFTs. As expected, FNet executed in PyTorch outperforms BERT executed in ONNX despite less framework overhead and numerous static optimizations -- with a 10.31\% speedup at batch size 1. For improvements in research frameworks to translate to deployment, additional investment can be directed towards support for complex control flow and operators in inference runtimes. 

\textbf{At large input sizes, framework and runtime overhead from graph operations is negligible.}
For batch sizes larger than 16, we find that there is minimal latency difference across models, inference runtimes, or execution frameworks. In this compute-bound regime, number of FLOPs is still a poor latency predictor due to variable execution time for different operations. For example, efficient mobile architectures that depend on invert-residual MBConv layers are memory inefficient and much slower per-FLOP than standard convolution and linear layers.

\textbf{For framework-bound models, model depth is a reasonable proxy for latency.}
Number of floating point operations is a poor indicator of latency in a framework-bound setting, as total runtime is generally constant and tied to framework overheads and the size of the computational graph. In framework-bound models, the size of the computational graph is related to model depth.

\textbf{Estimations of latency for models deployed in production settings must account for their target framework and hardware platform.}
Model development frequently occurs using eager execution research frameworks and hardware platforms. However, deployment often occurs in inference runtimes and on mobile devices or specialized inference hardware. This misalignment can mislead the development of ``efficient'' models that do not translate to real-world deployment settings. As such, researchers should be clear in specifying the ``efficiency" context, such as the target frameworks and hardware platform, when developing new methods. For example, techniques such as hardware-aware neural architecture search which leverage direct latency measures must also control for framework choices to account for this mismatch.
\begin{table}
\scriptsize
\centering
\begin{tabular}{@{}cccccc@{}}
\textbf{Self-Attn Dim} & \textbf{FC Dim} & \textbf{Batch} & \textbf{SeqLen} & \textbf{Latency} & \textbf{Throughput} \\ \toprule
\phantom{0}768 & 3072      & 1           & 128      & 0.0136    & 0.0136   \\ 
\phantom{0}768 & 3072      & 4           & 128      & 0.0134    & 0.0034   \\ 
\phantom{0}768 & 3072      & 1           & 512      & 0.0134    & 0.0134   \\ 
1536           & 6144      & 1           & 128      & 0.0134    & 0.0134   \\ 
\bottomrule
\end{tabular}
\caption{Latency of BERT PyTorch models on RTX-8000. Scaling along batch sizes and model width shows no increase in latency.}
\vspace{-15pt}
\label{tab:scaling-bert}
\end{table}

\textbf{Throughput and input size can be increased at no cost for framework-bound models.}
For a given model, latency is constant regardless of batch size until compute kernels saturate and exceed CPU launch costs. If computation for a particular input size is bottlenecked by framework overhead, the batch size or input size can be increased without increases in overall runtime. In practice, this can lead to the processing of larger batch sizes, sequence lengths, or higher image resolutions at no additional latency cost until kernel operations saturate framework overhead. See Table~\ref{tab:scaling-bert}.

\textbf{Model width can be increased at no cost for framework-bound models.}
For a given batch size, individual layers of a framework bound can be made wider by increasing hidden dimension or filter size without increases in latency. Wider models are known to exhibit better task performance due to increased parameter count and expressivity \cite{zagoruyko2016wide}.

Model designers can leverage wider architectures with their target inference framework and hardware setting in mind to achieve higher utilization. For example, models processing few examples during inference can leverage wider layers to avoid CPU framework bottlenecks. See Table~\ref{tab:scaling-bert}.

==> sections/6_futurework.tex <==
\section{Future Work}
While GPUs are the most common general purpose hardware accelerators, domain specific architectures such as Google TPU's, GraphCore IPUs, and custom ASICs present additional settings for future investigation. Likewise, we intend to extend our evaluations to other common frameworks and runtimes such as TensorFlow, Jax, TensorRT, and TVM.

As models continue to scale in size, they often require model or data parallelism techniques that require computation across several nodes which introduce overhead from multi-device synchronization and network communication. Additionally, we do not study latency in the training setting where the per-layer computation is larger due to the computation of gradients and losses.

 % Similarly, CUDA graphs present an exciting direction by offloading the cost of multiple kernel launches into the launch of a single fused computational graph.

==> sections/7_conclusions.tex <==
\section{Conclusion}
We conduct an extensive study of neural networks from the convolutional and transformer architecture paradigms across a variety of software and hardware platforms. We show that inference performed with these large neural networks, which was previously assumed to be compute bounded, is in fact limited by overhead incurred by deep learning frameworks. While wider transformer architectures (e.g. BERT-Base) exhibit less boundedness behaviors than narrower, deeper CNNs (e.g. ResNet-50), we show that all models exhibit framework boundedness.  Additionally, we observe that these inefficiencies are becoming more apparent as hardware accelerator speeds increase. 

We introduce the concept of the \textit{framework tax} to describe when improvements in hardware speed and reductions in required computation fail to translate to speedups in model latency and throughput due to bottlenecks incurred by deep learning frameworks. We hope that these observations raise awareness of the impact and limitations created by choice of framework on model development and deployment. 


% Hardware lottery=
% Through a comprehensive analysis of the machine learning inference hardware and software stack, we show that inference latency is most dependent on model architecture, frameworks, and underlying hardware platforms. 
% In contrast to model training, where gradient computation and workloads with large batch sizes saturate accelerators, inference latency is especially sensitive to CPU-side limitations in enqueueing high-quality kernels. We show that these limitations can bottleneck inference performance and introduce the new metric of framework overhead to analyze these bottlenecks. 

% We conducted an evaluation of model latency on GPUs across neural network framework paradigms and find that traditional efficiency cost indicators, such as number of FLOPs, model depth and parameter count are insufficient in characterizing a model's inference latency at all scales. We hope to elucidate a better understanding of efficiency and raise awareness of the various factors that affect inference performance to guide efficient model, framework, and hardware design.

==> sections/appx_hardware.tex <==

\section{Hardware Details}
\label{appx:hardware}
    Experiments were conducted on a slurm cluster with heterogeneous compute nodes. Compute node hardware details included in Table \ref{Tab:Hardware Platforms}.

    We use PyTorch 1.12.1 with CUDA 11.6 and Python 3.8.13. We use ONNX Runtime 1.7.0 with CUDA 11.1.1 and cuDNN v8.0.4.3. Baseline experiments are run on a compute node with an Nvidia RTX-8000 GPU and an Intel Xeon E5-2630 CPU with 32 GB of DDRAM memory.
    
\begin{table*}[H]
\footnotesize
\centering
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
\textbf{CPU} & \textbf{GPU}  & \textbf{GPU Arch} & \textbf{Core Count} & \textbf{Tensor Cores} & \textbf{Clock Rate (GHz)} & \textbf{Memory (GB)} & \textbf{Mem BW (GB/s)} & \textbf{FP16 TFLOPS} \\ 
\toprule
% \multirow{2}{*}{\textbf{CPU}}
% & \textbf{Xeon W-2295}	& Cascade Lake & 18 & - & 3.00 & 256 & 2.66 & 21.3 \\ \cline{2-9} 
% & \textbf{Cortex-A72} 	& Arm v8-A     & 4  & - & 1.50 & 8 	 & 2.8 & 3.95 \\ \hline
% \textbf{Intel Xeon E5-2630} & \textbf{Titan X}  	& Pascal  	& 3584 & - & 1.42 & 12 & 480.4 & 10.97 	\\ %\cline{2-9} 
\textbf{Intel Xeon Silver 4110} & \textbf{1080Ti} 	& Pascal  	& 3584 & - & 1.38 & 11 & 484.4 & 22.78  \\ %\cline{2-9} 
\textbf{Intel Xeon Gold 6242} & \textbf{V100}   	& Volta   	& 5120  & 640 & 1.23 & 32 & 897 & 28.26 \\ %\cline{2-9} 
\textbf{Intel Xeon E5-2630} & \textbf{2080Ti} 	& Turing	& 3584  & 544 & 1.35 & 11 & 616 & 26.90 \\ %\cline{2-9} 
\textbf{Intel Xeon E5-2630} & \textbf{\scriptsize{RTX-8000}}  & Turing	& 4608  & 576 & 1.40 & 48 & 672 & 32.62 \\ %\cline{2-9} 
\textbf{AMD EPYC 7282} & \textbf{3090}      & Ampere    & 10496 & 328 & 1.35 & 24 & 936 & 35.89 \\ %\cline{2-9} 
\textbf{Intel Xeon Silver 4110} & \textbf{A6000}     & Ampere    & 10752 & 336 & 1.41 & 48 & 768 & 38.71 \\ 
\textbf{Intel Xeon 8339HC} & \textbf{A100} & Ampere & 6912 & 432 & 1.215 & 40 & 1935 & 77.97\\
\bottomrule % change to midrule if you expect to do more platforms
\end{tabularx}
\caption{Detailed information on hardware platforms used throughout our experiments, in order of Nvidia  microarchitecture generation.  }
\label{Tab:Hardware Platforms}
\vspace{-10pt}
\end{table*}

==> sections/appx_implementation.tex <==
\appendix

	\textbf{Latency.} Inference latency is averaged over 100 forward passes of the model after a 10 iteration warm-up.
    
    \textbf{Memory Usage.} Max and average memory are measured with Nvidia NVML for GPU, and Python memory_profiler for CPU.
    
    \textbf{Number of Floating Point Operations.} 
    


==> sections/appx_operations.tex <==
\appendix
Case Studies
- Various ResNets
- 


Operations:
  - Factorized Operations
  - MBConvs 

  - Parallelised Execution

  - Reduction
  

==> sections/appx_verticals.tex <==
% \onecolumn

\section{Additional Figures}
\label{appx:figs}

% \begin{multicols}{2}

    % \begin{figure}[!ht]
    %         \centering
    %         \vspace{-10pt}
    %         \includegraphics[width=0.45\textwidth]{assets/assets-1/model_bs_latency.pdf}
    %         \vspace{-10pt}
    %         \caption{BERT and efficient variants on a 2080Ti. Efficient Transformer variants are slower than BERT at small batch sizes due to the introduction of more layers.} % TODO: Clean up this sentence
    %         % \vspace{-10pt}
    %         \label{fig:bs-efficient-bert}
    % \end{figure*}    
        
    % \begin{figure*}[!ht]
    %     \centering
    %     \includegraphics[width=0.45\textwidth]{assets/assets-1/throughput_gpu.pdf}
    %     \vspace{-5pt}
    %     \caption{BERT at different batch sizes on different hardware. At smaller batch sizes, faster GPU hardware does not increase throughput.} % TODO: Clean up this sentence
    %     \label{fig:throughput-gpu}
    % \end{figure*}    
    
    % \columnbreak
    \begin{figure*}[!ht]
            \centering
            \vspace{-10pt}
            \includegraphics[width=0.45\textwidth]{assets/assets-1/normalized_variance_batch.png}
            \vspace{-10pt}
            \caption{Framework boundedness is apparent at low batch sizes, as latency is consistent across accelerators. For larger models, framework boundedness dissipates for smaller bath sizes as inference becomes compute bound. Hardware used are the same as prior benchmarks.} % TODO: Clean up this sentence
            % \vspace{-10pt}
            \label{fig:fw-overhead-curve}
    \end{figure*}   
% \end{multicols}
